Integrating Reward Maximization and Population Estimation: Sequential Decision-Making for Internal Revenue Service Audit Selection

We introduce a new setting, optimize-and-estimate structured bandits. Here, a policy must select a batch of arms, each characterized by its own context, that would allow it to both maximize reward and maintain an accurate (ideally unbiased) population estimate of the reward. This setting is inherent to many public and private sector applications and often requires handling delayed feedback, small data, and distribution shifts. We demonstrate its importance on real data from the United States Internal Revenue Service (IRS). The IRS performs yearly audits of the tax base. Two of its most important objectives are to identify suspected misreporting and to estimate the "tax gap" -- the global difference between the amount paid and true amount owed. Based on a unique collaboration with the IRS, we cast these two processes as a unified optimize-and-estimate structured bandit. We analyze optimize-and-estimate approaches to the IRS problem and propose a novel mechanism for unbiased population estimation that achieves rewards comparable to baseline approaches. This approach has the potential to improve audit efficacy, while maintaining policy-relevant estimates of the tax gap. This has important social consequences given that the current tax gap is estimated at nearly half a trillion dollars. We suggest that this problem setting is fertile ground for further research and we highlight its interesting challenges. The results of this and related research are currently being incorporated into the continual improvement of the IRS audit selection methods.

==> aux-refs.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{bouneffouf2019survey}
\citation{henderson2021}
\citation{henderson2021,omb2018requirements,omb2021requirements}
\citation{sarin2019shrinking}
\providecommand \oddpage@label [2]{}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}\protected@file@percent }
\newlabel{submission}{{1}{1}{Introduction}{section.1}{}}
\citation{horvitz1952generalization}
\citation{bietti2018contextual}
\citation{bastani2021mostly}
\citation{guyton2021tax}
\citation{nie2018adaptively,xu2013estimation,shin2021bias}
\citation{dimakopoulou2017estimation}
\citation{liu2014trading,erraqabi2017trading}
\citation{abbasi2011improved,joseph2018meritocratic}
\citation{wagstaff2012machine}
\citation{gao2002new,gao2003irs}
\citation{andreoni1998tax,johns2010distribution,internal2016federal,internal2019federal}
\citation{marr2016irs,cbo2020trends}
\citation{internal2016federal,internal2019federal}
\citation{internal2019federal}
\citation{irm}
\citation{dif1976}
\citation{lawsky2008fairly}
\citation{andreoni1998tax,johns2010distribution,internal2016federal,internal2019federal}
\citation{belnap2020real}
\citation{guyton2018effects}
\citation{guyton2020tax,irs2012estimates,internal2016federal,internal2019federal}
\citation{erard2011individual}
\citation{tas2018improper}
\citation{omb2018requirements}
\citation{omb2021requirements}
\@writefile{toc}{\contentsline {section}{\numberline {2}Background}{3}{section.2}\protected@file@percent }
\newlabel{sec:background}{{2}{3}{Background}{section.2}{}}
\citation{nika2021contextual}
\citation{lattimore2020bandit}
\citation{esteban2019estimating}
\citation{lattimore2020bandit}
\citation{hutter2011sequential}
\@writefile{toc}{\contentsline {section}{\numberline {3}Methods}{4}{section.3}\protected@file@percent }
\citation{potter1990study,alexander1997making}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Illustration of ABS on 50 synthetic observations. (a) Hypothetical risk distribution and three parameterizations corresponding to different values of $\alpha $: 0.1, 1, and 5. Greedy selection, represented by the dotted (gray) line in each panel would choose the $K=10$ returns with the highest risk. The parameterized risk distributions are clustered into three strata ($S_1$, $S_2$, $S_3$), represented by the colored panels. As $\alpha $ varies, the cluster assignments change. (b) Probabilities of sampling a single individual from the three strata. As $\alpha $ increases, more weight is put onto the higher risk returns (Stratum 3). \relax }}{5}{figure.caption.2}\protected@file@percent }
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{fig:abs_sampling}{{1}{5}{Illustration of ABS on 50 synthetic observations. (a) Hypothetical risk distribution and three parameterizations corresponding to different values of $\alpha $: 0.1, 1, and 5. Greedy selection, represented by the dotted (gray) line in each panel would choose the $K=10$ returns with the highest risk. The parameterized risk distributions are clustered into three strata ($S_1$, $S_2$, $S_3$), represented by the colored panels. As $\alpha $ varies, the cluster assignments change. (b) Probabilities of sampling a single individual from the three strata. As $\alpha $ increases, more weight is put onto the higher risk returns (Stratum 3). \relax }{figure.caption.2}{}}
\@writefile{loa}{\contentsline {algorithm}{\numberline {1}{\ignorespaces ABS (Logistic)\relax }}{5}{figure.caption.3}\protected@file@percent }
\newlabel{alg:abs}{{1}{5}{ABS (Logistic)\relax }{figure.caption.3}{}}
\newlabel{eq:min_variance}{{3}{5}{Methods}{equation.3.3}{}}
\newlabel{eq:pi}{{4}{5}{Methods}{equation.3.4}{}}
\citation{bommasani2021opportunities}
\citation{lawsky2008fairly}
\citation{nochange,lederman2018does}
\citation{debacker2018effects}
\citation{nie2018adaptively,neel2018mitigating}
\@writefile{toc}{\contentsline {section}{\numberline {4}Evaluation Protocol}{6}{section.4}\protected@file@percent }
\newlabel{sec:eval}{{4}{6}{Evaluation Protocol}{section.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {5}Results}{6}{section.5}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {5.1}Unbiased population estimates are possible with little impact to reward}{6}{subsection.5.1}\protected@file@percent }
\citation{bietti2018contextual,kannan2018smoothed,bastani2021mostly}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces  Best settings with overlapping CIs ($^*$) on $R$. $R$ is a cumulative reward. $\mu _{PE}$ is the average percent difference of the population estimate across seeds. $\sigma _{PE}$ is the standard deviation of the percent difference across seeds. $\mu _{NR}$ is the no change rate. Extended table with hyperparameters for all displayed methods is in Appendix\nobreakspace  {}\ref  {app:allresults}, selection method in Appendix\nobreakspace  {}\ref  {app:hyperpararmeters}. Biased methods with no guarantees are highly undesirable ({\color  {red}{\fontfamily  {pzd}\fontencoding  {U}\fontseries  {m}\fontshape  {n}\selectfont  \char 55}}). $\epsilon $-only is the same as $\epsilon $-Greedy, but population estimation uses only the $\epsilon $ sample as a random sample. Random is where the full, 600 arm, sample is random. \relax }}{7}{table.caption.4}\protected@file@percent }
\newlabel{tab:best_reward}{{1}{7}{Best settings with overlapping CIs ($^*$) on $R$. $R$ is a cumulative reward. $\mu _{PE}$ is the average percent difference of the population estimate across seeds. $\sigma _{PE}$ is the standard deviation of the percent difference across seeds. $\mu _{NR}$ is the no change rate. Extended table with hyperparameters for all displayed methods is in Appendix~\ref {app:allresults}, selection method in Appendix~\ref {app:hyperpararmeters}. Biased methods with no guarantees are highly undesirable ({\color {red}\xmark }). $\eps $-only is the same as $\eps $-Greedy, but population estimation uses only the $\eps $ sample as a random sample. Random is where the full, 600 arm, sample is random. \relax }{table.caption.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.2}ABS allows fine-grained control over variance-reward trade-off}{7}{subsection.5.2}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces (Left) Population estimation empirical standard deviation versus reward for a grid of ABS hyperparameters. ({\color  {red}x}) and associated labels indicate $\epsilon $-only and fully random sample. (Right) Population estimation variance as a function of the trimming factor.\relax }}{7}{figure.caption.5}\protected@file@percent }
\newlabel{fig:variance}{{2}{7}{(Left) Population estimation empirical standard deviation versus reward for a grid of ABS hyperparameters. ({\color {red}x}) and associated labels indicate $\epsilon $-only and fully random sample. (Right) Population estimation variance as a function of the trimming factor.\relax }{figure.caption.5}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.3}Greedy is not all you need}{7}{subsection.5.3}\protected@file@percent }
\citation{bietti2018contextual,kannan2018smoothed,bastani2021mostly}
\citation{thrun1993issues,nie2018adaptively,shin2021bias,farquhar2021statistical}
\citation{lawsky2008fairly,davis2012unequal}
\citation{kiel,irs2021update,treasury2021american}
\citation{guyton2021tax}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces A kernel density plot of the distribution of sampled arms by reward from 2007, 2010, and 2014 (left to right, more in Appendix\nobreakspace  {}\ref  {app:allresults}). ``True'' refers to the density of all returns for the given year. X-axis is true reward. Y-axis is sampling distribution density.\relax }}{8}{figure.caption.6}\protected@file@percent }
\newlabel{fig:samplingdist}{{3}{8}{A kernel density plot of the distribution of sampled arms by reward from 2007, 2010, and 2014 (left to right, more in Appendix~\ref {app:allresults}). ``True'' refers to the density of all returns for the given year. X-axis is true reward. Y-axis is sampling distribution density.\relax }{figure.caption.6}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {5.4}A more focused approach audits higher cumulative total positive income}{8}{subsection.5.4}\protected@file@percent }
\newlabel{fig:income}{{4a}{9}{\relax }{figure.caption.7}{}}
\newlabel{sub@fig:income}{{a}{9}{\relax }{figure.caption.7}{}}
\newlabel{fig:income2}{{4b}{9}{\relax }{figure.caption.7}{}}
\newlabel{sub@fig:income2}{{b}{9}{\relax }{figure.caption.7}{}}
\newlabel{fig:classes}{{4c}{9}{\relax }{figure.caption.7}{}}
\newlabel{sub@fig:classes}{{c}{9}{\relax }{figure.caption.7}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces (a) The cumulative average total positive income (TPI) of all batches of taxpayers audited by each algorithm. (b) Across all ABS hyperparameters sampled, which allows fine-grained control over the population estimate variance and reward trade-off, the relationship between reward, no change rate, and cumulative average TPI. (c) The distribution of audit classes for several approaches. Top ABS selections are similar to RF Greedy, as shown separately in Appendix\nobreakspace  {}\ref  {app:allresults}. More details on labels for (c) are provided in Appendix\nobreakspace  {}\ref  {app:more_data}. \relax }}{9}{figure.caption.7}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {5.5}Errors are heteroskedastic, causing difficulties in using model-based optimism methods}{9}{subsection.5.5}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {6}Discussion}{9}{section.6}\protected@file@percent }
\bibstyle{plainnat}
\bibdata{main}
\bibcite{abbasi2011improved}{{1}{2011}{{Abbasi-Yadkori et~al.}}{{Abbasi-Yadkori, P{\'a}l, and Szepesv{\'a}ri}}}
\bibcite{abe1999associative}{{2}{1999}{{Abe and Long}}{{}}}
\bibcite{agarwal2021deep}{{3}{2021}{{Agarwal et~al.}}{{Agarwal, Schwarzer, Castro, Courville, and Bellemare}}}
\bibcite{agrawal2015linear}{{4}{2015}{{Agrawal and Devanur}}{{}}}
\bibcite{alexander1997making}{{5}{1997}{{Alexander et~al.}}{{Alexander, Dahl, and Weidman}}}
\bibcite{andreoni1998tax}{{6}{1998}{{Andreoni et~al.}}{{Andreoni, Erard, and Feinstein}}}
\bibcite{ash2021machine}{{7}{2021}{{Ash et~al.}}{{Ash, Galletta, and Giommoni}}}
\bibcite{bastani2021mostly}{{8}{2021}{{Bastani et~al.}}{{Bastani, Bayati, and Khosravi}}}
\bibcite{nochange}{{9}{2015}{{Beer et~al.}}{{Beer, Kasper, Kirchler, and Erard}}}
\bibcite{belnap2020real}{{10}{2020}{{Belnap et~al.}}{{Belnap, Hoopes, Maydew, and Turk}}}
\bibcite{bertomeu2021using}{{11}{2021}{{Bertomeu et~al.}}{{Bertomeu, Cheynel, Floyd, and Pan}}}
\bibcite{biecek2018dalex}{{12}{2018}{{Biecek}}{{}}}
\bibcite{bietti2018contextual}{{13}{2018}{{Bietti et~al.}}{{Bietti, Agarwal, and Langford}}}
\bibcite{bommasani2021opportunities}{{14}{2021}{{Bommasani et~al.}}{{Bommasani, Hudson, Adeli, Altman, Arora, von Arx, Bernstein, Bohg, Bosselut, Brunskill, et~al.}}}
\bibcite{bouneffouf2019survey}{{15}{2019}{{Bouneffouf and Rish}}{{}}}
\bibcite{bouthillier2021accounting}{{16}{2021}{{Bouthillier et~al.}}{{Bouthillier, Delaunay, Bronzi, Trofimov, Nichyporuk, Szeto, Mohammadi~Sepahvand, Raff, Madan, Voleti, et~al.}}}
\bibcite{caria2020adaptive}{{17}{2020}{{Caria et~al.}}{{Caria, Kasy, Quinn, Shami, Teytelboym, et~al.}}}
\bibcite{chugg2021reconciling}{{18}{2021}{{Chugg and Ho}}{{}}}
\bibcite{cbo2020trends}{{19}{2020}{{Congressional Budget Office}}{{}}}
\bibcite{davis2012unequal}{{20}{2012}{{Davis-Nozemack}}{{}}}
\bibcite{de2018tax}{{21}{2018}{{de~Roux et~al.}}{{de~Roux, Perez, Moreno, Villamil, and Figueroa}}}
\bibcite{debacker2015importing}{{22}{2015}{{DeBacker et~al.}}{{DeBacker, Heim, and Tran}}}
\bibcite{debacker2018effects}{{23}{2018}{{DeBacker et~al.}}{{DeBacker, Heim, Tran, and Yuskavage}}}
\bibcite{deliu2021efficient}{{24}{2021}{{Deliu et~al.}}{{Deliu, Williams, and Villar}}}
\bibcite{dickey2019machine}{{25}{2019}{{Dickey et~al.}}{{Dickey, Blanke, and Seaton}}}
\bibcite{dimakopoulou2017estimation}{{26}{2017}{{Dimakopoulou et~al.}}{{Dimakopoulou, Zhou, Athey, and Imbens}}}
\bibcite{drugan2014scalarization}{{27}{2014}{{Drugan and Now{\'e}}}{{}}}
\bibcite{dularif2019deterrence}{{28}{2019}{{Dularif et~al.}}{{Dularif, Sutrisno, Saraswati, et~al.}}}
\bibcite{erard2011individual}{{29}{2011}{{Erard and Feinstein}}{{}}}
\bibcite{erraqabi2017trading}{{30}{2017}{{Erraqabi et~al.}}{{Erraqabi, Lazaric, Valko, Brunskill, and Liu}}}
\bibcite{esteban2019estimating}{{31}{2019}{{Esteban et~al.}}{{Esteban, McRoberts, Fern{\'a}ndez-Landa, Tom{\'e}, and N{\ae }sset}}}
\bibcite{farquhar2021statistical}{{32}{2021}{{Farquhar et~al.}}{{Farquhar, Gal, and Rainforth}}}
\bibcite{foster2020beyond}{{33}{2020}{{Foster and Rakhlin}}{{}}}
\bibcite{foster2020instance}{{34}{2020}{{Foster et~al.}}{{Foster, Rakhlin, Simchi-Levi, and Xu}}}
\bibcite{gao2002new}{{35}{2002}{{Government Accountability Office}}{{}}}
\bibcite{gao2003irs}{{36}{2003}{{Government Accountability Office}}{{}}}
\bibcite{guo2021learning}{{37}{2021}{{Guo et~al.}}{{Guo, Agrawal, Grover, Muthukumar, and Pananjady}}}
\bibcite{guyton2018effects}{{38}{2018}{{Guyton et~al.}}{{Guyton, Leibel, Manoli, Patel, Payne, and Schafer}}}
\bibcite{guyton2020tax}{{39}{2020}{{Guyton et~al.}}{{Guyton, Langetieg, Reck, Risch, and Zucman}}}
\bibcite{guyton2021tax}{{40}{2021}{{Guyton et~al.}}{{Guyton, Langetieg, Reck, Risch, and Zucman}}}
\bibcite{henderson2018deep}{{41}{2018}{{Henderson et~al.}}{{Henderson, Islam, Bachman, Pineau, Precup, and Meger}}}
\bibcite{henderson2020towards}{{42}{2020}{{Henderson et~al.}}{{Henderson, Hu, Romoff, Brunskill, Jurafsky, and Pineau}}}
\bibcite{henderson2021}{{43}{2021}{{{Henderson} et~al.}}{{{Henderson}, {Chugg}, {Anderson}, and {Ho}}}}
\bibcite{ho2020affirmative}{{44}{2020}{{Ho and Xiang}}{{}}}
\bibcite{horvitz1952generalization}{{45}{1952}{{Horvitz and Thompson}}{{}}}
\bibcite{howard2020can}{{46}{2020}{{Howard et~al.}}{{Howard, Lykke, Pinski, and Plumley}}}
\bibcite{huang2016linear}{{47}{2016}{{Huang and Lin}}{{}}}
\bibcite{hutter2011sequential}{{48}{2011}{{Hutter et~al.}}{{Hutter, Hoos, and Leyton-Brown}}}
\bibcite{irs2012estimates}{{49}{2012}{{Internal Revenue Service}}{{}}}
\bibcite{internal2016federal}{{50}{2016}{{Internal Revenue Service}}{{}}}
\bibcite{internal2019federal}{{51}{2019}{{Internal Revenue Service}}{{}}}
\bibcite{irs2021update}{{52}{2021}{{Internal Revenue Service}}{{}}}
\bibcite{irm}{{53}{2022}{{Internal Revenue Service}}{{}}}
\bibcite{jarvelin2002cumulated}{{54}{2002}{{J{\"a}rvelin and Kek{\"a}l{\"a}inen}}{{}}}
\bibcite{johns2010distribution}{{55}{2010}{{Johns and Slemrod}}{{}}}
\bibcite{joseph2018meritocratic}{{56}{2018}{{Joseph et~al.}}{{Joseph, Kearns, Morgenstern, Neel, and Roth}}}
\bibcite{kannan2018smoothed}{{57}{2018}{{Kannan et~al.}}{{Kannan, Morgenstern, Roth, Waggoner, and Wu}}}
\bibcite{kasy2021adaptive}{{58}{2021}{{Kasy and Sautmann}}{{}}}
\bibcite{katerenchuk2018rankdcg}{{59}{2018}{{Katerenchuk and Rosenberg}}{{}}}
\bibcite{kato2020efficient}{{60}{2020}{{Kato et~al.}}{{Kato, Ishihara, Honda, and Narita}}}
\bibcite{kiel}{{61}{2019}{{Kiel}}{{}}}
\bibcite{kotsiantis2006predicting}{{62}{2006}{{Kotsiantis et~al.}}{{Kotsiantis, Koumanakos, Tzelepis, and Tampakas}}}
\bibcite{lacoste2019quantifying}{{63}{2019}{{Lacoste et~al.}}{{Lacoste, Luccioni, Schmidt, and Dandres}}}
\bibcite{lansdell2019rarely}{{64}{2019}{{Lansdell et~al.}}{{Lansdell, Triantafillou, and Kording}}}
\bibcite{lattimore2020bandit}{{65}{2020}{{Lattimore and Szepesv{\'a}ri}}{{}}}
\bibcite{lawsky2008fairly}{{66}{2008}{{Lawsky}}{{}}}
\bibcite{lederman2018does}{{67}{2018}{{Lederman}}{{}}}
\bibcite{li2010contextual}{{68}{2010}{{Li et~al.}}{{Li, Chu, Langford, and Schapire}}}
\bibcite{liu2014trading}{{69}{2014}{{Liu et~al.}}{{Liu, Mandel, Brunskill, and Popovic}}}
\bibcite{dif1976}{{70}{1976}{{Lowe}}{{}}}
\bibcite{marr2016irs}{{71}{2016}{{Marr and Murray}}{{}}}
\bibcite{latenonfiler}{{72}{2016}{{Matta et~al.}}{{Matta, Guyton, Hodge~II, Langetieg, Orlett, Payne, Qadri, Rupert, Schafer, Turk, and Vigil}}}
\bibcite{mersereau2009structured}{{73}{2009}{{Mersereau et~al.}}{{Mersereau, Rusmevichientong, and Tsitsiklis}}}
\bibcite{mittal2018bogus}{{74}{2018}{{Mittal et~al.}}{{Mittal, Reich, and Mahajan}}}
\bibcite{mukherjee2020generalized}{{75}{2020}{{Mukherjee et~al.}}{{Mukherjee, Tripathy, and Nowak}}}
\bibcite{neel2018mitigating}{{76}{2018}{{Neel and Roth}}{{}}}
\bibcite{nie2018adaptively}{{77}{2018}{{Nie et~al.}}{{Nie, Tian, Taylor, and Zou}}}
\bibcite{nika2021contextual}{{78}{2021}{{Nika et~al.}}{{Nika, Elahi, and Tekin}}}
\bibcite{omb2018requirements}{{79}{2018}{{Office of Management and Budget}}{{}}}
\bibcite{omb2021requirements}{{80}{2021}{{Office of Management and Budget}}{{}}}
\bibcite{pandey2006handling}{{81}{2006}{{Pandey and Olston}}{{}}}
\bibcite{politis2003impact}{{82}{2003}{{Politis}}{{}}}
\bibcite{politis1994large}{{83}{1994}{{Politis and Romano}}{{}}}
\bibcite{politisromanoj}{{84}{1999}{{Politis et~al.}}{{Politis, Romano, and Wolf}}}
\bibcite{potter1990study}{{85}{1990}{{Potter}}{{}}}
\bibcite{qin2022adaptivity}{{86}{2022}{{Qin and Russo}}{{}}}
\bibcite{rafferty2018bandit}{{87}{2018}{{Rafferty et~al.}}{{Rafferty, Ying, and Williams}}}
\bibcite{sarin2019shrinking}{{88}{2019}{{Sarin and Summers}}{{}}}
\bibcite{sen2021top}{{89}{2021}{{Sen et~al.}}{{Sen, Rakhlin, Ying, Kidambi, Foster, Hill, and Dhillon}}}
\bibcite{sener2018active}{{90}{2018}{{Sener and Savarese}}{{}}}
\bibcite{settles2009active}{{91}{2009}{{Settles}}{{}}}
\bibcite{shao1989general}{{92}{1989}{{Shao and Wu}}{{}}}
\bibcite{shin2021bias}{{93}{2021}{{Shin et~al.}}{{Shin, Ramdas, and Rinaldo}}}
\bibcite{sifa2019towards}{{94}{2019}{{Sifa et~al.}}{{Sifa, Ladi, Pielka, Ramamurthy, Hillebrand, Kirsch, Biesner, Stenzel, Bell, L{"u}bbering, et~al.}}}
\bibcite{simchi2020bypassing}{{95}{2020}{{Simchi-Levi and Xu}}{{}}}
\bibcite{slemrod2019tax}{{96}{2019}{{Slemrod}}{{}}}
\bibcite{snow2005tax}{{97}{2005}{{Snow and Warren~Jr}}{{}}}
\bibcite{soemers2018adapting}{{98}{2018}{{Soemers et~al.}}{{Soemers, Brys, Driessens, Winands, and Now{\'e}}}}
\bibcite{tas2018improper}{{99}{2018}{{Taxpayer Advocate Service}}{{}}}
\bibcite{tekin2018multi}{{100}{2018}{{Tekin and Tur{\u {g}}ay}}{{}}}
\bibcite{thrun1993issues}{{101}{1993}{{Thrun and Schwartz}}{{}}}
\bibcite{treasury2021american}{{102}{2021}{{Treasury}}{{}}}
\bibcite{turgay2018multi}{{103}{2018}{{Turgay et~al.}}{{Turgay, Oner, and Tekin}}}
\bibcite{pums}{{104}{2018}{{United States Census Bureau}}{{}}}
\bibcite{asec}{{105}{2019}{{United States Census Bureau}}{{}}}
\bibcite{wagstaff2012machine}{{106}{2012}{{Wagstaff}}{{}}}
\bibcite{webb2016characterizing}{{107}{2016}{{Webb et~al.}}{{Webb, Hyde, Cao, Nguyen, and Petitjean}}}
\bibcite{wortman2007maintaining}{{108}{2007}{{Wortman et~al.}}{{Wortman, Vorobeychik, Li, and Langford}}}
\bibcite{xiang2020reconciling}{{109}{2020}{{Xiang}}{{}}}
\bibcite{xu2013estimation}{{110}{2013}{{Xu et~al.}}{{Xu, Qin, and Liu}}}
\bibcite{zhang2020inference}{{111}{2020}{{Zhang et~al.}}{{Zhang, Janson, and Murphy}}}
\bibcite{zheng2020ai}{{112}{2020}{{Zheng et~al.}}{{Zheng, Trott, Srinivasa, Naik, Gruesbeck, Parkes, and Socher}}}
\bibcite{zhu2022contextual}{{113}{2022}{{Zhu et~al.}}{{Zhu, Foster, Langford, and Mineiro}}}
\citation{pums}
\citation{asec}
\citation{lacoste2019quantifying}
\citation{henderson2020towards}
\citation{treasury2021american}
\citation{henderson2021}
\citation{xiang2020reconciling,ho2020affirmative}
\@writefile{toc}{\contentsline {section}{\numberline {A}Software and Data}{18}{appendix.A}\protected@file@percent }
\newlabel{app:code}{{A}{18}{Software and Data}{appendix.A}{}}
\@writefile{toc}{\contentsline {section}{\numberline {B}Carbon Impact Statement}{18}{appendix.B}\protected@file@percent }
\newlabel{app:carbon}{{B}{18}{Carbon Impact Statement}{appendix.B}{}}
\@writefile{toc}{\contentsline {section}{\numberline {C}Society/Ethics Statement}{18}{appendix.C}\protected@file@percent }
\newlabel{app:ethics}{{C}{18}{Society/Ethics Statement}{appendix.C}{}}
\citation{deliu2021efficient}
\citation{caria2020adaptive}
\citation{kasy2021adaptive}
\citation{pandey2006handling}
\citation{xu2013estimation}
\citation{guo2021learning}
\citation{dimakopoulou2017estimation}
\citation{qin2022adaptivity}
\citation{sen2021top}
\citation{simchi2020bypassing}
\citation{huang2016linear}
\citation{abbasi2011improved}
\citation{joseph2018meritocratic}
\citation{dickey2019machine,bertomeu2021using}
\citation{de2018tax}
\citation{kotsiantis2006predicting}
\citation{sifa2019towards}
\citation{soemers2018adapting}
\citation{zheng2020ai}
\citation{howard2020can,ash2021machine,mittal2018bogus}
\citation{drugan2014scalarization,tekin2018multi,turgay2018multi}
\citation{mersereau2009structured,abbasi2011improved,joseph2018meritocratic}
\citation{sen2021top}
\citation{huang2016linear}
\citation{li2010contextual}
\citation{li2010contextual}
\citation{huang2016linear}
\citation{agrawal2015linear}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces For clarity, we provide a comparison against related work.\relax }}{19}{table.caption.12}\protected@file@percent }
\newlabel{tab:rwork}{{2}{19}{For clarity, we provide a comparison against related work.\relax }{table.caption.12}{}}
\@writefile{toc}{\contentsline {section}{\numberline {D}Related Work}{19}{appendix.D}\protected@file@percent }
\newlabel{sec:related_work}{{D}{19}{Related Work}{appendix.D}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {D.1}Similar Applications}{19}{subsection.D.1}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {D.2}Multi-objective Decision-making}{19}{subsection.D.2}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {D.3}Batch Selection}{19}{subsection.D.3}\protected@file@percent }
\citation{shin2021bias,nie2018adaptively,xu2013estimation}
\citation{kato2020efficient,mukherjee2020generalized,deliu2021efficient}
\citation{kasy2021adaptive,wortman2007maintaining,zhang2020inference,lansdell2019rarely}
\citation{dimakopoulou2017estimation}
\citation{chugg2021reconciling}
\citation{guo2021learning}
\citation{pandey2006handling,wortman2007maintaining,xu2013estimation}
\citation{liu2014trading,rafferty2018bandit}
\citation{caria2020adaptive}
\citation{erraqabi2017trading}
\citation{deliu2021efficient}
\citation{caria2020adaptive}
\citation{settles2009active}
\citation{joseph2018meritocratic}
\citation{abbasi2011improved}
\citation{joseph2018meritocratic}
\citation{abbasi2011improved}
\@writefile{toc}{\contentsline {subsection}{\numberline {D.4}Inference}{20}{subsection.D.4}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {D.5}Active Learning}{20}{subsection.D.5}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {D.6}Discussion}{20}{subsection.D.6}\protected@file@percent }
\citation{caria2020adaptive}
\citation{lattimore2020bandit}
\citation{slemrod2019tax,snow2005tax}
\citation{dularif2019deterrence}
\@writefile{toc}{\contentsline {section}{\numberline {E}Baseline Methods Selection}{21}{appendix.E}\protected@file@percent }
\newlabel{app:baselines}{{E}{21}{Baseline Methods Selection}{appendix.E}{}}
\@writefile{toc}{\contentsline {section}{\numberline {F}Limitations}{21}{appendix.F}\protected@file@percent }
\newlabel{app:limitations}{{F}{21}{Limitations}{appendix.F}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {F.1}Deterrence}{21}{subsection.F.1}\protected@file@percent }
\newlabel{app:deterrence}{{F.1}{21}{Deterrence}{subsection.F.1}{}}
\citation{omb2018requirements}
\citation{omb2018requirements}
\citation{biecek2018dalex}
\citation{webb2016characterizing}
\@writefile{toc}{\contentsline {section}{\numberline {G}Importance and Relevance of the Optimize-and-Estimate Setting}{22}{appendix.G}\protected@file@percent }
\newlabel{app:relevance}{{G}{22}{Importance and Relevance of the Optimize-and-Estimate Setting}{appendix.G}{}}
\@writefile{toc}{\contentsline {section}{\numberline {H}Covariate Drift}{22}{appendix.H}\protected@file@percent }
\newlabel{app:drift}{{H}{22}{Covariate Drift}{appendix.H}{}}
\@writefile{toc}{\contentsline {section}{\numberline {I}More Data Details}{23}{appendix.I}\protected@file@percent }
\newlabel{app:more_data}{{I}{23}{More Data Details}{appendix.I}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces We illustrate the current tax audit process. As described in Section\nobreakspace  {}\ref  {sec:background}, the NRP audits are jointly used for population estimation of non-compliance and risk model training. The Op audits are then selected from the DIF model but are never used for estimating the tax gap or for re-training the DIF risk model.\relax }}{23}{figure.caption.13}\protected@file@percent }
\newlabel{fig:IRS_overview}{{5}{23}{We illustrate the current tax audit process. As described in Section~\ref {sec:background}, the NRP audits are jointly used for population estimation of non-compliance and risk model training. The Op audits are then selected from the DIF model but are never used for estimating the tax gap or for re-training the DIF risk model.\relax }{figure.caption.13}{}}
\@writefile{lot}{\contentsline {table}{\numberline {3}{\ignorespaces Correspondence between structured bandit framework and our setting.\relax }}{23}{table.caption.14}\protected@file@percent }
\newlabel{tab:irs_bandit}{{3}{23}{Correspondence between structured bandit framework and our setting.\relax }{table.caption.14}{}}
\@writefile{lot}{\contentsline {table}{\numberline {4}{\ignorespaces Summary statistics by year of the average misreporting per audited taxpayer across the NRP sample. $\mu $-uw is unweighted mean, $\mu $-w is the mean weighted by NRP sample weights. Cov. drift is the year-over-year covariate drift. No change is the no change rate. $\DOTSB \sum@ \slimits@ w$ is the sum of the NRP sample weights for a given year, equal to the total sampling population.\relax }}{23}{table.caption.15}\protected@file@percent }
\newlabel{tab:NRP}{{4}{23}{Summary statistics by year of the average misreporting per audited taxpayer across the NRP sample. $\mu $-uw is unweighted mean, $\mu $-w is the mean weighted by NRP sample weights. Cov. drift is the year-over-year covariate drift. No change is the no change rate. $\sum w$ is the sum of the NRP sample weights for a given year, equal to the total sampling population.\relax }{table.caption.15}{}}
\@writefile{lot}{\contentsline {table}{\numberline {5}{\ignorespaces Counts for each NRP class by year in the full NRP sample.\relax }}{24}{table.caption.16}\protected@file@percent }
\newlabel{tab:classcounts}{{5}{24}{Counts for each NRP class by year in the full NRP sample.\relax }{table.caption.16}{}}
\@writefile{lot}{\contentsline {table}{\numberline {6}{\ignorespaces A correspondence of audit classes to their descriptions. Replicated from \url {https://www.irs.gov/pub/irs-pia/2018_doc_6209_section_13.pdf}. TGR is Sch. C/F Total Gross Receipts (TGR). TPI is total positive income. Schedule F is a form filed with tax returns used to report Profit or Loss From Farming. Schedule C is used to report income or loss from a business operated or a profession practiced as a sole proprietor. Schedule E is used to ``report income or loss from rental real estate, royalties, partnerships, S corporations, estates, trusts, and residual interests in real estate mortgage investment conduits (REMICs).'' See \url {https://www.irs.gov/forms-pubs/about-schedule-e-form-1040}. Form 2106 is used to report business expenses. See \url {https://www.irs.gov/forms-pubs/about-form-2106}. EITC is the Earned Income Tax Credit for low-to-moderate-income families and workers. See \url {https://www.irs.gov/credits-deductions/individuals/earned-income-tax-credit-eitc}. \relax }}{24}{table.caption.17}\protected@file@percent }
\newlabel{tab:auditclass_desc}{{6}{24}{A correspondence of audit classes to their descriptions. Replicated from \protect \url {https://www.irs.gov/pub/irs-pia/2018_doc_6209_section_13.pdf}. TGR is Sch. C/F Total Gross Receipts (TGR). TPI is total positive income. Schedule F is a form filed with tax returns used to report Profit or Loss From Farming. Schedule C is used to report income or loss from a business operated or a profession practiced as a sole proprietor. Schedule E is used to ``report income or loss from rental real estate, royalties, partnerships, S corporations, estates, trusts, and residual interests in real estate mortgage investment conduits (REMICs).'' See \protect \url {https://www.irs.gov/forms-pubs/about-schedule-e-form-1040}. Form 2106 is used to report business expenses. See \protect \url {https://www.irs.gov/forms-pubs/about-form-2106}. EITC is the Earned Income Tax Credit for low-to-moderate-income families and workers. See \protect \url {https://www.irs.gov/credits-deductions/individuals/earned-income-tax-credit-eitc}. \relax }{table.caption.17}{}}
\@writefile{toc}{\contentsline {section}{\numberline {J}NRP Weights}{24}{appendix.J}\protected@file@percent }
\newlabel{app:nrp_weights}{{J}{24}{NRP Weights}{appendix.J}{}}
\citation{henderson2018deep,agarwal2021deep}
\citation{jarvelin2002cumulated}
\citation{katerenchuk2018rankdcg}
\citation{jarvelin2002cumulated,katerenchuk2018rankdcg}
\@writefile{toc}{\contentsline {section}{\numberline {K}Extended Metrics Descriptions}{25}{appendix.K}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {K.1}Choice of cumulative versus average Reward and Total Positive Income}{25}{subsection.K.1}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {K.2}Extended Percent Difference Explanation}{25}{subsection.K.2}\protected@file@percent }
\newlabel{app:pd}{{K.2}{25}{Extended Percent Difference Explanation}{subsection.K.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {K.3}RARE Score}{25}{subsection.K.3}\protected@file@percent }
\newlabel{app:rare}{{K.3}{25}{RARE Score}{subsection.K.3}{}}
\citation{horvitz1952generalization}
\@writefile{toc}{\contentsline {section}{\numberline {L}Function Approximator Selection}{26}{appendix.L}\protected@file@percent }
\newlabel{app:functionapproximator}{{L}{26}{Function Approximator Selection}{appendix.L}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces RARE score for linear versus non-linear methods, with non-linear achieving significantly improved performance, especially at higher budgets. ``lin-e'' refers to a linear (ridge regression with regularization factor of 1.0) $\epsilon $-greedy model, ``ols-e'' to an ordinary least squares (no regularization) $\epsilon $-greedy model, and ``rf-e'' to a random forest $\epsilon $-greedy model. Here we plot 30 runs with standard errors. \relax }}{26}{figure.caption.18}\protected@file@percent }
\newlabel{fig:function_approximators}{{6}{26}{RARE score for linear versus non-linear methods, with non-linear achieving significantly improved performance, especially at higher budgets. ``lin-e'' refers to a linear (ridge regression with regularization factor of 1.0) $\eps $-greedy model, ``ols-e'' to an ordinary least squares (no regularization) $\eps $-greedy model, and ``rf-e'' to a random forest $\eps $-greedy model. Here we plot 30 runs with standard errors. \relax }{figure.caption.18}{}}
\@writefile{toc}{\contentsline {section}{\numberline {M}ABS Sampling}{26}{appendix.M}\protected@file@percent }
\newlabel{app:abs_sampling}{{M}{26}{ABS Sampling}{appendix.M}{}}
\newlabel{eq:min_variance1}{{6}{26}{ABS Sampling}{equation.M.6}{}}
\newlabel{eq:pi1}{{7}{26}{ABS Sampling}{equation.M.7}{}}
\@writefile{loa}{\contentsline {algorithm}{\numberline {2}{\ignorespaces Adaptive Bin Sampling - Logistic Smoothing\relax }}{27}{algorithm.2}\protected@file@percent }
\newlabel{alg:abs2}{{2}{27}{Adaptive Bin Sampling - Logistic Smoothing\relax }{algorithm.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {M.1}Variance of Population Estimate}{27}{subsection.M.1}\protected@file@percent }
\citation{henderson2020towards}
\citation{henderson2018deep,bouthillier2021accounting,agarwal2021deep}
\citation{joseph2018meritocratic}
\@writefile{toc}{\contentsline {section}{\numberline {N}Experimental Setup}{29}{appendix.N}\protected@file@percent }
\newlabel{app:expsetup2}{{N}{29}{Experimental Setup}{appendix.N}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Diagram describing our experimental setup.\relax }}{29}{figure.caption.19}\protected@file@percent }
\newlabel{fig:processdiagram}{{7}{29}{Diagram describing our experimental setup.\relax }{figure.caption.19}{}}
\@writefile{toc}{\contentsline {section}{\numberline {O}Hyperparameter Tuning}{29}{appendix.O}\protected@file@percent }
\newlabel{app:hyperpararmeters}{{O}{29}{Hyperparameter Tuning}{appendix.O}{}}
\@writefile{lot}{\contentsline {table}{\numberline {7}{\ignorespaces Hyperparameter grids\relax }}{29}{table.caption.20}\protected@file@percent }
\newlabel{tab:hparamgrid}{{7}{29}{Hyperparameter grids\relax }{table.caption.20}{}}
\citation{latenonfiler}
\citation{debacker2015importing}
\citation{sener2018active}
\citation{sener2018active}
\citation{politis1994large,politisromanoj,politis2003impact}
\citation{politisromanoj,shao1989general}
\@writefile{toc}{\contentsline {section}{\numberline {P}Winsorization}{30}{appendix.P}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\numberline {Q}Budget Selection}{30}{appendix.Q}\protected@file@percent }
\newlabel{app:budgets}{{Q}{30}{Budget Selection}{appendix.Q}{}}
\@writefile{toc}{\contentsline {section}{\numberline {R}Confidence Intervals on the Time Series}{30}{appendix.R}\protected@file@percent }
\newlabel{app:confidenceintervals}{{R}{30}{Confidence Intervals on the Time Series}{appendix.R}{}}
\@writefile{toc}{\contentsline {section}{\numberline {S}Results}{31}{appendix.S}\protected@file@percent }
\newlabel{app:allresults}{{S}{31}{Results}{appendix.S}{}}
\@writefile{lot}{\contentsline {table}{\numberline {8}{\ignorespaces We rank all methods and hyperparameters based on reward bands. We show the top reward band and best hyperparameter settings for each method in that reward band (where CIs across random seeds overlap). $R$ is the average cumulative reward at the final timestep across random seeds, $\mu _{NR}$ is the average no-change rate, $\mu _{RARE}$ the average RARE score, $\mu _{PE}$ the absolute percent difference of the population estimate, and $\sigma _{PE}$ the standard deviation of the population estimate. $\sqrt  {|\mu _{PE}|_2^2}$ is root mean squared error.\relax }}{31}{table.caption.21}\protected@file@percent }
\newlabel{tab:best_reward_app}{{8}{31}{We rank all methods and hyperparameters based on reward bands. We show the top reward band and best hyperparameter settings for each method in that reward band (where CIs across random seeds overlap). $R$ is the average cumulative reward at the final timestep across random seeds, $\mu _{NR}$ is the average no-change rate, $\mu _{RARE}$ the average RARE score, $\mu _{PE}$ the absolute percent difference of the population estimate, and $\sigma _{PE}$ the standard deviation of the population estimate. $\sqrt {|\mu _{PE}|_2^2}$ is root mean squared error.\relax }{table.caption.21}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.1}$\epsilon $-Greedy, Random Sample-Only for Population Estimation}{31}{subsection.S.1}\protected@file@percent }
\newlabel{app:eps}{{S.1}{31}{$\eps $-Greedy, Random Sample-Only for Population Estimation}{subsection.S.1}{}}
\@writefile{lot}{\contentsline {table}{\numberline {9}{\ignorespaces The population estimation variance across random seeds and reward given different amounts of $\epsilon $-Greedy exploration samples.\relax }}{31}{table.caption.22}\protected@file@percent }
\newlabel{tab:eps-only}{{9}{31}{The population estimation variance across random seeds and reward given different amounts of $\eps $-Greedy exploration samples.\relax }{table.caption.22}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.2}Price-for-variance Trade-offs and Policy Implications}{31}{subsection.S.2}\protected@file@percent }
\newlabel{app:pricemetric}{{S.2}{31}{Price-for-variance Trade-offs and Policy Implications}{subsection.S.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces The pareto front of ABS hyperparameters with a cubic fit. This can be thought of as the marginal benefit for giving up reward.\relax }}{32}{figure.caption.23}\protected@file@percent }
\newlabel{fig:marginal}{{8}{32}{The pareto front of ABS hyperparameters with a cubic fit. This can be thought of as the marginal benefit for giving up reward.\relax }{figure.caption.23}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.3}Using RFR significantly outperforms LDA and incorporating non-random data helps}{32}{subsection.S.3}\protected@file@percent }
\newlabel{app:lda}{{S.3}{32}{Using RFR significantly outperforms LDA and incorporating non-random data helps}{subsection.S.3}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces A comparison of cumulative reward earned between LDA-based approaches and RFR-based approaches. FRO indicates that the RFR was fit to the random sample only.\relax }}{33}{figure.caption.24}\protected@file@percent }
\newlabel{fig:lda}{{9}{33}{A comparison of cumulative reward earned between LDA-based approaches and RFR-based approaches. FRO indicates that the RFR was fit to the random sample only.\relax }{figure.caption.24}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.4}Fine-grained Kernel Density}{33}{subsection.S.4}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces A kernel density plot of the distribution of sampled arms from 2006 (top left) to 2014 (bottom). X-axis is true reward. Y-axis is sampling distribution density.\relax }}{33}{figure.caption.25}\protected@file@percent }
\newlabel{fig:samplingdist2}{{10}{33}{A kernel density plot of the distribution of sampled arms from 2006 (top left) to 2014 (bottom). X-axis is true reward. Y-axis is sampling distribution density.\relax }{figure.caption.25}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.5}Ablation of ABS}{33}{subsection.S.5}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces Results for ABS with a budget of 600 arms. The top row explores the effect of $\zeta $ on five metrics, the middle row explores the effect of $\alpha $, and the bottom the effect of the trimming factor.\relax }}{34}{figure.caption.26}\protected@file@percent }
\newlabel{fig:abs_results}{{11}{34}{Results for ABS with a budget of 600 arms. The top row explores the effect of $\zeta $ on five metrics, the middle row explores the effect of $\alpha $, and the bottom the effect of the trimming factor.\relax }{figure.caption.26}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.6}Larger Budget}{34}{subsection.S.6}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces Results for ABS with a budget of 1000 arms. The top row explores the effect of $\zeta $ (Z) on five metrics, the middle row explores the effect of $\alpha $, and the bottom the effect of the trimming factor.\relax }}{34}{figure.caption.27}\protected@file@percent }
\newlabel{fig:abs_results1000}{{12}{34}{Results for ABS with a budget of 1000 arms. The top row explores the effect of $\zeta $ (Z) on five metrics, the middle row explores the effect of $\alpha $, and the bottom the effect of the trimming factor.\relax }{figure.caption.27}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {S.7}Sampling breakdown by classes}{34}{subsection.S.7}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\numberline {S.8}Expanded Figure}{34}{subsection.S.8}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {13}{\ignorespaces Top Left, Middle, Right: ABS hyperparameters with a budget of 1000 arms. Trends largely reflect results at the budget of 600 arms. Bottom: similarly, cumulative rewards for greedy and UCB methods follow trends as in the 600 budget setting.\relax }}{35}{figure.caption.28}\protected@file@percent }
\newlabel{fig:more_results1000}{{13}{35}{Top Left, Middle, Right: ABS hyperparameters with a budget of 1000 arms. Trends largely reflect results at the budget of 600 arms. Bottom: similarly, cumulative rewards for greedy and UCB methods follow trends as in the 600 budget setting.\relax }{figure.caption.28}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {14}{\ignorespaces Top: Comparison of the top ABS hyperparameter settings seen in Table\nobreakspace  {}\ref  {tab:best_reward} with RF $\epsilon $-greedy as a reference. Bottom: A small ablation of $\zeta $'s effect on class selection counts for an ABS setting of logistic mixing function, $\alpha =0.5$ and a 5\% trim. \relax }}{35}{figure.caption.29}\protected@file@percent }
\newlabel{fig:moreclass}{{14}{35}{Top: Comparison of the top ABS hyperparameter settings seen in Table~\ref {tab:best_reward} with RF $\epsilon $-greedy as a reference. Bottom: A small ablation of $\zeta $'s effect on class selection counts for an ABS setting of logistic mixing function, $\alpha =0.5$ and a 5\% trim. \relax }{figure.caption.29}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {15}{\ignorespaces For clarity we include a non-log scale version of Figure\nobreakspace  {}\ref  {fig:variance} results and compare it with the other version.\relax }}{36}{figure.caption.30}\protected@file@percent }
\newlabel{fig:exp2fig}{{15}{36}{For clarity we include a non-log scale version of Figure~\ref {fig:variance} results and compare it with the other version.\relax }{figure.caption.30}{}}
\@input{proof.aux}
\relax 
\providecommand\hyper@newdestlabel[2]{}
\citation{sen2021top}
\citation{simchi2020bypassing}
\citation{sen2021top}
\citation{sen2021top}
\citation{abe1999associative}
\citation{foster2020beyond,simchi2020bypassing,foster2020instance,sen2021top,zhu2022contextual}
\citation{sen2021top}
\citation{sen2021top}
\citation{simchi2020bypassing}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\@writefile{toc}{\contentsline {section}{\numberline {T}Regret}{37}{appendix.T}\protected@file@percent }
\newlabel{app:regret}{{T}{37}{Regret}{appendix.T}{}}
\citation{sen2021top}
\newlabel{eq:abs_mixture}{{{8}}{38}{Regret}{AMS.32}{}}
\newlabel{eq:functionalform}{{{9}}{38}{Regret}{AMS.34}{}}
\newlabel{lem:abs_bound}{{1}{38}{ABS Minimum Probability Bound}{lemma.1}{}}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\newlabel{asum:realizability}{{1}{39}{\bf Realizability}{assumption.1}{}}
\newlabel{thm:topkregret}{{1}{39}{}{theorem.1}{}}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\newlabel{lem:square_prob_bound}{{2}{40}{}{lemma.2}{}}
\newlabel{lem:blorg}{{3}{40}{}{lemma.3}{}}
\citation{sen2021top}
\newlabel{eq:twoparthing}{{{12}}{42}{Regret}{AMS.36}{}}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\@writefile{toc}{\contentsline {paragraph}{Induction hypothesis ($\tau $):}{43}{section*.37}\protected@file@percent }
\newlabel{eq:reg_decompose}{{{13}}{43}{Induction hypothesis ($\tau $):}{AMS.39}{}}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\newlabel{eq:RemplessR}{{14}{44}{Induction hypothesis ($\tau $):}{equation.T.14}{}}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\citation{sen2021top}
\newlabel{lem:fhat_bound}{{4}{45}{}{lemma.4}{}}
\citation{sen2021top}
\@setckpt{proof}{
\setcounter{page}{48}
\setcounter{equation}{20}
\setcounter{enumi}{5}
\setcounter{enumii}{3}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{9}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{section}{20}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{15}
\setcounter{table}{9}
\setcounter{NAT@ctr}{113}
\setcounter{parentequation}{0}
\setcounter{float@type}{8}
\setcounter{algorithm}{2}
\setcounter{ALC@line}{16}
\setcounter{ALC@rem}{16}
\setcounter{caption@flags}{0}
\setcounter{continuedfloat}{0}
\setcounter{subfigure}{0}
\setcounter{subtable}{0}
\setcounter{cp@cntr}{0}
\setcounter{Item}{23}
\setcounter{Hfootnote}{9}
\setcounter{bookmark@seq@number}{50}
\setcounter{theorem}{1}
\setcounter{example}{0}
\setcounter{property}{0}
\setcounter{lemma}{4}
\setcounter{proposition}{0}
\setcounter{remark}{0}
\setcounter{corollary}{0}
\setcounter{definition}{0}
\setcounter{conjecture}{0}
\setcounter{claim}{0}
\setcounter{assumption}{1}
\setcounter{section@level}{4}
}


==> defs.tex <==

\RequirePackage{xpatch}

\xpatchcmd{\proof}{\itshape}{\normalfont\proofnameformat}{}{}
\newcommand{\proofnameformat}{\bfseries}



\RequirePackage{latexsym}
\RequirePackage{amsmath}
\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{stmaryrd}
\RequirePackage{environ}

\makeatletter
\@ifpackageloaded{dsfont}{}{\newcommand{\mathds}[1]{\mathbb{#1}}}
\@ifpackageloaded{mathrsfs}{}{\newcommand{\mathscr}[1]{\mathcal{#1}}}
\makeatother






\newcommand{\ab}{{\bm{a}}}
\newcommand{\bb}{{\bm{b}}}
\newcommand{\cbb}{{\bm{c}}}
\newcommand{\db}{{\bm{d}}}
\newcommand{\eb}{{\bm{e}}}
\newcommand{\fb}{{\bm{f}}}
\newcommand{\gb}{{\bm{g}}}
\newcommand{\hb}{{\bm{h}}}
\newcommand{\ib}{{\bm{i}}}
\newcommand{\jb}{{\bm{j}}}
\newcommand{\kb}{{\bm{k}}}
\newcommand{\lb}{{\bm{l}}}
\newcommand{\mb}{{\bm{m}}}
\newcommand{\nbb}{{\bm{n}}}
\newcommand{\ob}{{\bm{o}}}
\newcommand{\qb}{{\bm{q}}}
\newcommand{\rb}{{\bm{r}}}
\newcommand{\sbb}{{\bm{s}}}
\newcommand{\tb}{{\bm{t}}}
\newcommand{\ub}{{\bm{u}}}
\newcommand{\wb}{{\bm{w}}}
\newcommand{\xb}{{\bm{x}}}
\newcommand{\yb}{{\bm{y}}}
\newcommand{\zb}{{\bm{z}}}

\newcommand{\ba}{\ab}
\newcommand{\bc}{\cbb}
\newcommand{\bd}{\db}
\newcommand{\be}{\eb}
\newcommand{\bbf}{\fb}
\newcommand{\bff}{\fb}
\newcommand{\bg}{\gb}
\newcommand{\bh}{\hb}
\newcommand{\bi}{\ib}
\newcommand{\bj}{\jb}
\newcommand{\bk}{\kb}
\newcommand{\bl}{\lb}
\newcommand{\bbm}{\mb}
\newcommand{\bmm}{\mb}
\newcommand{\bn}{\nbb}
\newcommand{\bo}{\ob}
\newcommand{\bp}{\pb}
\newcommand{\bq}{\qb}
\newcommand{\br}{\rb}
\newcommand{\bs}{\sbb}
\newcommand{\bt}{\tb}
\newcommand{\bu}{\ub}
\newcommand{\bv}{\vb}
\newcommand{\bw}{\wb}
\newcommand{\bx}{\xb}
\newcommand{\by}{\yb}
\newcommand{\bz}{\zb}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\at}{\tilde{a}}
\newcommand{\bti}{\tilde{b}}
\newcommand{\ct}{\tilde{c}}
\newcommand{\dt}{\tilde{d}}
\newcommand{\et}{\tilde{e}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\gt}{\tilde{g}}
\newcommand{\hti}{\tilde{h}}
\newcommand{\htt}{\tilde{h}}
\newcommand{\iti}{\tilde{i}}
\newcommand{\itt}{\tilde{i}}
\newcommand{\jt}{\tilde{j}}
\newcommand{\kt}{\tilde{k}}
\newcommand{\lt}{\tilde{l}}
\newcommand{\mt}{\tilde{m}}
\newcommand{\nt}{\tilde{n}}
\newcommand{\ot}{\tilde{o}}
\newcommand{\pti}{\tilde{p}}
\newcommand{\ptt}{\tilde{p}}
\newcommand{\qt}{\tilde{q}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\st}{\tilde{s}}
\newcommand{\tti}{\tilde{t}}
\newcommand{\ttt}{\tilde{t}}
\newcommand{\ut}{\tilde{u}}
\newcommand{\vti}{\tilde{v}}
\newcommand{\vtt}{\tilde{v}}
\newcommand{\wt}{\tilde{w}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\yt}{\tilde{y}}
\newcommand{\zt}{\tilde{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\batil}{\tilde{\ab}}
\newcommand{\bctil}{\tilde{\cbb}}
\newcommand{\bdtil}{\tilde{\db}}
\newcommand{\betil}{\tilde{\eb}}
\newcommand{\bftil}{\tilde{\fb}}
\newcommand{\bgtil}{\tilde{\gb}}
\newcommand{\bhtil}{\tilde{\hb}}
\newcommand{\bitil}{\tilde{\ib}}
\newcommand{\bjtil}{\tilde{\jb}}
\newcommand{\bktil}{\tilde{\kb}}
\newcommand{\bltil}{\tilde{\lb}}
\newcommand{\bmtil}{\tilde{\mb}}
\newcommand{\bntil}{\tilde{\nbb}}
\newcommand{\botil}{\tilde{\ob}}
\newcommand{\bptil}{\tilde{\pb}}
\newcommand{\bqtil}{\tilde{\qb}}
\newcommand{\brtil}{\tilde{\rb}}
\newcommand{\bstil}{\tilde{\sbb}}
\newcommand{\bttil}{\tilde{\tb}}
\newcommand{\butil}{\tilde{\ub}}
\newcommand{\bvtil}{\tilde{\vb}}
\newcommand{\bwtil}{\tilde{\wb}}
\newcommand{\bxtil}{\tilde{\xb}}
\newcommand{\bytil}{\tilde{\yb}}
\newcommand{\bztil}{\tilde{\zb}}

\newcommand{\bat}{\tilde{\ab}}
\newcommand{\bbt}{\tilde{\bb}}
\newcommand{\bct}{\tilde{\cbb}}
\newcommand{\bdt}{\tilde{\db}}
\newcommand{\bet}{\tilde{\eb}}
\newcommand{\bft}{\tilde{\fb}}
\newcommand{\bgt}{\tilde{\gb}}
\newcommand{\bht}{\tilde{\hb}}
\newcommand{\bit}{\tilde{\ib}}
\newcommand{\bjt}{\tilde{\jb}}
\newcommand{\bkt}{\tilde{\kb}}
\newcommand{\blt}{\tilde{\lb}}
\newcommand{\bmt}{\tilde{\mb}}
\newcommand{\bnt}{\tilde{\nbb}}
\newcommand{\boti}{\tilde{\ob}}
\newcommand{\boot}{\tilde{\ob}}
\newcommand{\bpt}{\tilde{\pb}}
\newcommand{\bqt}{\tilde{\qb}}
\newcommand{\brt}{\tilde{\rb}}
\newcommand{\bst}{\tilde{\sbb}}
\newcommand{\btti}{\tilde{\tb}}
\newcommand{\btt}{\tilde{\tb}}
\newcommand{\but}{\tilde{\ub}}
\newcommand{\bvt}{\tilde{\vb}}
\newcommand{\bwt}{\tilde{\wb}}
\newcommand{\bxt}{\tilde{\xb}}
\newcommand{\byt}{\tilde{\yb}}
\newcommand{\bzt}{\tilde{\zb}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\bahat}{\hat{\ab}}
\newcommand{\bchat}{\hat{\bc}}
\newcommand{\bdhat}{\hat{\db}}
\newcommand{\behat}{\hat{\eb}}
\newcommand{\bfhat}{\hat{\fb}}
\newcommand{\bghat}{\hat{\gb}}
\newcommand{\bhhat}{\hat{\hb}}
\newcommand{\bihat}{\hat{\ib}}
\newcommand{\bjhat}{\hat{\jb}}
\newcommand{\bkhat}{\hat{\kb}}
\newcommand{\blhat}{\hat{\lb}}
\newcommand{\bmhat}{\hat{\mb}}
\newcommand{\bnhat}{\hat{\nbb}}
\newcommand{\bohat}{\hat{\ob}}
\newcommand{\bphat}{\hat{\pb}}
\newcommand{\bqhat}{\hat{\qb}}
\newcommand{\brhat}{\hat{\rb}}
\newcommand{\bshat}{\hat{\sbb}}
\newcommand{\bthat}{\hat{\tb}}
\newcommand{\buhat}{\hat{\ub}}
\newcommand{\bvhat}{\hat{\vb}}
\newcommand{\bwhat}{\hat{\wb}}
\newcommand{\bxhat}{\hat{\xb}}
\newcommand{\byhat}{\hat{\yb}}
\newcommand{\bzhat}{\hat{\zb}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obr}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\babar}{\bar{\ab}}
\newcommand{\bcbar}{\bar{\bc}}
\newcommand{\bdbar}{\bar{\db}}
\newcommand{\bebar}{\bar{\eb}}
\newcommand{\bfbar}{\bar{\fb}}
\newcommand{\bgbar}{\bar{\gb}}
\newcommand{\bhbar}{\bar{\hb}}
\newcommand{\bibar}{\bar{\ib}}
\newcommand{\bjbar}{\bar{\jb}}
\newcommand{\bkbar}{\bar{\kb}}
\newcommand{\blbar}{\bar{\lb}}
\newcommand{\bmbar}{\bar{\mb}}
\newcommand{\bnbar}{\bar{\nbb}}
\newcommand{\bobar}{\bar{\ob}}
\newcommand{\bpbar}{\bar{\pb}}
\newcommand{\bqbar}{\bar{\qb}}
\newcommand{\brbar}{\bar{\rb}}
\newcommand{\bsbar}{\bar{\sbb}}
\newcommand{\btbar}{\bar{\tb}}
\newcommand{\bubar}{\bar{\ub}}
\newcommand{\bvbar}{\bar{\vb}}
\newcommand{\bwbar}{\bar{\wb}}
\newcommand{\bxbar}{\bar{\xb}}
\newcommand{\bybar}{\bar{\yb}}
\newcommand{\bzbar}{\bar{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\At}{\tilde{A}}
\newcommand{\Bt}{\tilde{B}}
\newcommand{\Ct}{\tilde{C}}
\newcommand{\Dt}{\tilde{D}}
\newcommand{\Et}{\tilde{E}}
\newcommand{\Ft}{\tilde{F}}
\newcommand{\Gt}{\tilde{G}}
\newcommand{\Ht}{\tilde{H}}
\newcommand{\It}{\tilde{I}}
\newcommand{\Jt}{\tilde{J}}
\newcommand{\Kt}{\tilde{K}}
\newcommand{\Lt}{\tilde{L}}
\newcommand{\Mt}{\tilde{M}}
\newcommand{\Nt}{\tilde{N}}
\newcommand{\Ot}{\tilde{O}}
\newcommand{\Pt}{\tilde{P}}
\newcommand{\Qt}{\tilde{Q}}
\newcommand{\Rt}{\tilde{R}}
\newcommand{\St}{\tilde{S}}
\newcommand{\Tt}{\tilde{T}}
\newcommand{\Ut}{\tilde{U}}
\newcommand{\Vt}{\tilde{V}}
\newcommand{\Wt}{\tilde{W}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Zt}{\tilde{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Ab}{\bm{{A}}}
\newcommand{\Bb}{\bm{{B}}}
\newcommand{\Cb}{\bm{{C}}}
\newcommand{\Db}{\bm{{D}}}
\newcommand{\Eb}{\bm{{E}}}
\newcommand{\Fb}{\bm{{F}}}
\newcommand{\Gb}{\bm{{G}}}
\newcommand{\Hb}{\bm{{H}}}
\newcommand{\Ib}{\bm{{I}}}
\newcommand{\Jb}{\bm{{J}}}
\newcommand{\Kb}{\bm{{K}}}
\newcommand{\Lb}{\bm{{L}}}
\newcommand{\Mb}{\bm{{M}}}
\newcommand{\Nb}{\bm{{N}}}
\newcommand{\Ob}{\bm{{O}}}
\newcommand{\Pb}{\bm{{P}}}
\newcommand{\Qb}{\bm{{Q}}}
\newcommand{\Rb}{\bm{{R}}}
\newcommand{\Sbb}{\bm{{S}}}
\newcommand{\Tb}{\bm{{T}}}
\newcommand{\Ub}{\bm{{U}}}
\newcommand{\Vb}{\bm{{V}}}
\newcommand{\Wb}{\bm{{W}}}
\newcommand{\Xb}{\bm{{X}}}
\newcommand{\Yb}{\bm{{Y}}}
\newcommand{\Zb}{\bm{{Z}}}

\newcommand{\bA}{\bm{{A}}}
\newcommand{\bB}{\bm{{B}}}
\newcommand{\bC}{\bm{{C}}}
\newcommand{\bD}{\bm{{D}}}
\newcommand{\bE}{\bm{{E}}}
\newcommand{\bF}{\bm{{F}}}
\newcommand{\bG}{\bm{{G}}}
\newcommand{\bH}{\bm{{H}}}
\newcommand{\bI}{\bm{{I}}}
\newcommand{\bJ}{\bm{{J}}}
\newcommand{\bK}{\bm{{K}}}
\newcommand{\bL}{\bm{{L}}}
\newcommand{\bM}{\bm{{M}}}
\newcommand{\bN}{\bm{{N}}}
\newcommand{\bO}{\bm{{O}}}
\newcommand{\bP}{\bm{{P}}}
\newcommand{\bQ}{\bm{{Q}}}
\newcommand{\bR}{\bm{{R}}}
\newcommand{\bS}{\bm{{S}}}
\newcommand{\bT}{\bm{{T}}}
\newcommand{\bU}{\bm{{U}}}
\newcommand{\bV}{\bm{{V}}}
\newcommand{\bW}{\bm{{W}}}
\newcommand{\bX}{\bm{{X}}}
\newcommand{\bY}{\bm{{Y}}}
\newcommand{\bZ}{\bm{{Z}}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\bAt}{\tilde{\Ab}}
\newcommand{\bBt}{\tilde{\Bb}}
\newcommand{\bCt}{\tilde{\Cb}}
\newcommand{\bDt}{\tilde{\Db}}
\newcommand{\bEt}{\tilde{\Eb}}
\newcommand{\bFt}{\tilde{\Fb}}
\newcommand{\bGt}{\tilde{\Gb}}
\newcommand{\bHt}{\tilde{\Hb}}
\newcommand{\bIt}{\tilde{\Ib}}
\newcommand{\bJt}{\tilde{\Jb}}
\newcommand{\bKt}{\tilde{\Kb}}
\newcommand{\bLt}{\tilde{\Lb}}
\newcommand{\bMt}{\tilde{\Mb}}
\newcommand{\bNt}{\tilde{\Nb}}
\newcommand{\bOt}{\tilde{\Ob}}
\newcommand{\bPt}{\tilde{\Pb}}
\newcommand{\bQt}{\tilde{\Qb}}
\newcommand{\bRt}{\tilde{\Rb}}
\newcommand{\bSt}{\tilde{\Sbb}}
\newcommand{\bTt}{\tilde{\Tb}}
\newcommand{\bUt}{\tilde{\Ub}}
\newcommand{\bVt}{\tilde{\Vb}}
\newcommand{\bWt}{\tilde{\Wb}}
\newcommand{\bXt}{\tilde{\Xb}}
\newcommand{\bYt}{\tilde{\Yb}}
\newcommand{\bZt}{\tilde{\Zb}}

\newcommand{\bAtil}{\tilde{\Ab}}
\newcommand{\bBtil}{\tilde{\Bb}}
\newcommand{\bCtil}{\tilde{\Cb}}
\newcommand{\bDtil}{\tilde{\Db}}
\newcommand{\bEtil}{\tilde{\Eb}}
\newcommand{\bFtil}{\tilde{\Fb}}
\newcommand{\bGtil}{\tilde{\Gb}}
\newcommand{\bHtil}{\tilde{\Hb}}
\newcommand{\bItil}{\tilde{\Ib}}
\newcommand{\bJtil}{\tilde{\Jb}}
\newcommand{\bKtil}{\tilde{\Kb}}
\newcommand{\bLtil}{\tilde{\Lb}}
\newcommand{\bMtil}{\tilde{\Mb}}
\newcommand{\bNtil}{\tilde{\Nb}}
\newcommand{\bOtil}{\tilde{\Ob}}
\newcommand{\bPtil}{\tilde{\Pb}}
\newcommand{\bQtil}{\tilde{\Qb}}
\newcommand{\bRtil}{\tilde{\Rb}}
\newcommand{\bStil}{\tilde{\Sbb}}
\newcommand{\bTtil}{\tilde{\Tb}}
\newcommand{\bUtil}{\tilde{\Ub}}
\newcommand{\bVtil}{\tilde{\Vb}}
\newcommand{\bWtil}{\tilde{\Wb}}
\newcommand{\bXtil}{\tilde{\Xb}}
\newcommand{\bYtil}{\tilde{\Yb}}
\newcommand{\bZtil}{\tilde{\Zb}}

\newcommand{\bAtilde}{\widetilde{\Ab}}
\newcommand{\bBtilde}{\widetilde{\Bb}}
\newcommand{\bCtilde}{\widetilde{\Cb}}
\newcommand{\bDtilde}{\widetilde{\Db}}
\newcommand{\bEtilde}{\widetilde{\Eb}}
\newcommand{\bFtilde}{\widetilde{\Fb}}
\newcommand{\bGtilde}{\widetilde{\Gb}}
\newcommand{\bHtilde}{\widetilde{\Hb}}
\newcommand{\bItilde}{\widetilde{\Ib}}
\newcommand{\bJtilde}{\widetilde{\Jb}}
\newcommand{\bKtilde}{\widetilde{\Kb}}
\newcommand{\bLtilde}{\widetilde{\Lb}}
\newcommand{\bMtilde}{\widetilde{\Mb}}
\newcommand{\bNtilde}{\widetilde{\Nb}}
\newcommand{\bOtilde}{\widetilde{\Ob}}
\newcommand{\bPtilde}{\widetilde{\Pb}}
\newcommand{\bQtilde}{\widetilde{\Qb}}
\newcommand{\bRtilde}{\widetilde{\Rb}}
\newcommand{\bStilde}{\widetilde{\Sbb}}
\newcommand{\bTtilde}{\widetilde{\Tb}}
\newcommand{\bUtilde}{\widetilde{\Ub}}
\newcommand{\bVtilde}{\widetilde{\Vb}}
\newcommand{\bWtilde}{\widetilde{\Wb}}
\newcommand{\bXtilde}{\widetilde{\Xb}}
\newcommand{\bYtilde}{\widetilde{\Yb}}
\newcommand{\bZtilde}{\widetilde{\Zb}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sbb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\bAbar}{\bar{\Ab}}
\newcommand{\bBbar}{\bar{\Bb}}
\newcommand{\bCbar}{\bar{\Cb}}
\newcommand{\bDbar}{\bar{\Db}}
\newcommand{\bEbar}{\bar{\Eb}}
\newcommand{\bFbar}{\bar{\Fb}}
\newcommand{\bGbar}{\bar{\Gb}}
\newcommand{\bHbar}{\bar{\Hb}}
\newcommand{\bIbar}{\bar{\Ib}}
\newcommand{\bJbar}{\bar{\Jb}}
\newcommand{\bKbar}{\bar{\Kb}}
\newcommand{\bLbar}{\bar{\Lb}}
\newcommand{\bMbar}{\bar{\Mb}}
\newcommand{\bNbar}{\bar{\Nb}}
\newcommand{\bObar}{\bar{\Ob}}
\newcommand{\bPbar}{\bar{\Pb}}
\newcommand{\bQbar}{\bar{\Qb}}
\newcommand{\bRbar}{\bar{\Rb}}
\newcommand{\bSbar}{\bar{\Sbb}}
\newcommand{\bTbar}{\bar{\Tb}}
\newcommand{\bUbar}{\bar{\Ub}}
\newcommand{\bVbar}{\bar{\Vb}}
\newcommand{\bWbar}{\bar{\Wb}}
\newcommand{\bXbar}{\bar{\Xb}}
\newcommand{\bYbar}{\bar{\Yb}}
\newcommand{\bZbar}{\bar{\Zb}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sbb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\bAhat}{\hat{\Ab}}
\newcommand{\bBhat}{\hat{\Bb}}
\newcommand{\bChat}{\hat{\Cb}}
\newcommand{\bDhat}{\hat{\Db}}
\newcommand{\bEhat}{\hat{\Eb}}
\newcommand{\bFhat}{\hat{\Fb}}
\newcommand{\bGhat}{\hat{\Gb}}
\newcommand{\bHhat}{\hat{\Hb}}
\newcommand{\bIhat}{\hat{\Ib}}
\newcommand{\bJhat}{\hat{\Jb}}
\newcommand{\bKhat}{\hat{\Kb}}
\newcommand{\bLhat}{\hat{\Lb}}
\newcommand{\bMhat}{\hat{\Mb}}
\newcommand{\bNhat}{\hat{\Nb}}
\newcommand{\bOhat}{\hat{\Ob}}
\newcommand{\bPhat}{\hat{\Pb}}
\newcommand{\bQhat}{\hat{\Qb}}
\newcommand{\bRhat}{\hat{\Rb}}
\newcommand{\bShat}{\hat{\Sbb}}
\newcommand{\bThat}{\hat{\Tb}}
\newcommand{\bUhat}{\hat{\Ub}}
\newcommand{\bVhat}{\hat{\Vb}}
\newcommand{\bWhat}{\hat{\Wb}}
\newcommand{\bXhat}{\hat{\Xb}}
\newcommand{\bYhat}{\hat{\Yb}}
\newcommand{\bZhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\Acaltil}{\tilde{\cA}}
\newcommand{\Bcaltil}{\tilde{\cB}}
\newcommand{\Ccaltil}{\tilde{\cC}}
\newcommand{\Dcaltil}{\tilde{\cD}}
\newcommand{\Ecaltil}{\tilde{\cE}}
\newcommand{\Fcaltil}{\tilde{\cF}}
\newcommand{\Gcaltil}{\tilde{\cG}}
\newcommand{\Hcaltil}{\tilde{\cH}}
\newcommand{\Icaltil}{\tilde{\cI}}
\newcommand{\Jcaltil}{\tilde{\cJ}}
\newcommand{\Kcaltil}{\tilde{\cK}}
\newcommand{\Lcaltil}{\tilde{\cL}}
\newcommand{\Mcaltil}{\tilde{\cM}}
\newcommand{\Ncaltil}{\tilde{\cN}}
\newcommand{\Ocaltil}{\tilde{\cO}}
\newcommand{\Pcaltil}{\tilde{\cP}}
\newcommand{\Qcaltil}{\tilde{\cQ}}
\newcommand{\Rcaltil}{\tilde{\cR}}
\newcommand{\Scaltil}{\tilde{\cS}}
\newcommand{\Tcaltil}{\tilde{\cT}}
\newcommand{\Ucaltil}{\tilde{\cU}}
\newcommand{\Vcaltil}{\tilde{\cV}}
\newcommand{\Wcaltil}{\tilde{\cW}}
\newcommand{\Xcaltil}{\tilde{\cX}}
\newcommand{\Ycaltil}{\tilde{\cY}}
\newcommand{\Zcaltil}{\tilde{\cZ}}

\newcommand{\cAtil}{\tilde{\cA}}
\newcommand{\cBtil}{\tilde{\cB}}
\newcommand{\cCtil}{\tilde{\cC}}
\newcommand{\cDtil}{\tilde{\cD}}
\newcommand{\cEtil}{\tilde{\cE}}
\newcommand{\cFtil}{\tilde{\cF}}
\newcommand{\cGtil}{\tilde{\cG}}
\newcommand{\cHtil}{\tilde{\cH}}
\newcommand{\cItil}{\tilde{\cI}}
\newcommand{\cJtil}{\tilde{\cJ}}
\newcommand{\cKtil}{\tilde{\cK}}
\newcommand{\cLtil}{\tilde{\cL}}
\newcommand{\cMtil}{\tilde{\cM}}
\newcommand{\cNtil}{\tilde{\cN}}
\newcommand{\cOtil}{\tilde{\cO}}
\newcommand{\cPtil}{\tilde{\cP}}
\newcommand{\cQtil}{\tilde{\cQ}}
\newcommand{\cRtil}{\tilde{\cR}}
\newcommand{\cStil}{\tilde{\cS}}
\newcommand{\cTtil}{\tilde{\cT}}
\newcommand{\cUtil}{\tilde{\cU}}
\newcommand{\cVtil}{\tilde{\cV}}
\newcommand{\cWtil}{\tilde{\cW}}
\newcommand{\cXtil}{\tilde{\cX}}
\newcommand{\cYtil}{\tilde{\cY}}
\newcommand{\cZtil}{\tilde{\cZ}}

\newcommand{\cAt}{\tilde{\cA}}
\newcommand{\cBt}{\tilde{\cB}}
\newcommand{\cCt}{\tilde{\cC}}
\newcommand{\cDt}{\tilde{\cD}}
\newcommand{\cEt}{\tilde{\cE}}
\newcommand{\cFt}{\tilde{\cF}}
\newcommand{\cGt}{\tilde{\cG}}
\newcommand{\cHt}{\tilde{\cH}}
\newcommand{\cIt}{\tilde{\cI}}
\newcommand{\cJt}{\tilde{\cJ}}
\newcommand{\cKt}{\tilde{\cK}}
\newcommand{\cLt}{\tilde{\cL}}
\newcommand{\cMt}{\tilde{\cM}}
\newcommand{\cNt}{\tilde{\cN}}
\newcommand{\cOt}{\tilde{\cO}}
\newcommand{\cPt}{\tilde{\cP}}
\newcommand{\cQt}{\tilde{\cQ}}
\newcommand{\cRt}{\tilde{\cR}}
\newcommand{\cSt}{\tilde{\cS}}
\newcommand{\cTt}{\tilde{\cT}}
\newcommand{\cUt}{\tilde{\cU}}
\newcommand{\cVt}{\tilde{\cV}}
\newcommand{\cWt}{\tilde{\cW}}
\newcommand{\cXt}{\tilde{\cX}}
\newcommand{\cYt}{\tilde{\cY}}
\newcommand{\cZt}{\tilde{\cZ}}

\newcommand{\cAtilde}{\widetilde{\cA}}
\newcommand{\cBtilde}{\widetilde{\cB}}
\newcommand{\cCtilde}{\widetilde{\cC}}
\newcommand{\cDtilde}{\widetilde{\cD}}
\newcommand{\cEtilde}{\widetilde{\cE}}
\newcommand{\cFtilde}{\widetilde{\cF}}
\newcommand{\cGtilde}{\widetilde{\cG}}
\newcommand{\cHtilde}{\widetilde{\cH}}
\newcommand{\cItilde}{\widetilde{\cI}}
\newcommand{\cJtilde}{\widetilde{\cJ}}
\newcommand{\cKtilde}{\widetilde{\cK}}
\newcommand{\cLtilde}{\widetilde{\cL}}
\newcommand{\cMtilde}{\widetilde{\cM}}
\newcommand{\cNtilde}{\widetilde{\cN}}
\newcommand{\cOtilde}{\widetilde{\cO}}
\newcommand{\cPtilde}{\widetilde{\cP}}
\newcommand{\cQtilde}{\widetilde{\cQ}}
\newcommand{\cRtilde}{\widetilde{\cR}}
\newcommand{\cStilde}{\widetilde{\cS}}
\newcommand{\cTtilde}{\widetilde{\cT}}
\newcommand{\cUtilde}{\widetilde{\cU}}
\newcommand{\cVtilde}{\widetilde{\cV}}
\newcommand{\cWtilde}{\widetilde{\cW}}
\newcommand{\cXtilde}{\widetilde{\cX}}
\newcommand{\cYtilde}{\widetilde{\cY}}
\newcommand{\cZtilde}{\widetilde{\cZ}}

\newcommand{\Acalhat}{\hat{\cA}}
\newcommand{\Bcalhat}{\hat{\cB}}
\newcommand{\Ccalhat}{\hat{\cC}}
\newcommand{\Dcalhat}{\hat{\cD}}
\newcommand{\Ecalhat}{\hat{\cE}}
\newcommand{\Fcalhat}{\hat{\cF}}
\newcommand{\Gcalhat}{\hat{\cG}}
\newcommand{\Hcalhat}{\hat{\cH}}
\newcommand{\Icalhat}{\hat{\cI}}
\newcommand{\Jcalhat}{\hat{\cJ}}
\newcommand{\Kcalhat}{\hat{\cK}}
\newcommand{\Lcalhat}{\hat{\cL}}
\newcommand{\Mcalhat}{\hat{\cM}}
\newcommand{\Ncalhat}{\hat{\cN}}
\newcommand{\Ocalhat}{\hat{\cO}}
\newcommand{\Pcalhat}{\hat{\cP}}
\newcommand{\Qcalhat}{\hat{\cQ}}
\newcommand{\Rcalhat}{\hat{\cR}}
\newcommand{\Scalhat}{\hat{\cS}}
\newcommand{\Tcalhat}{\hat{\cT}}
\newcommand{\Ucalhat}{\hat{\cU}}
\newcommand{\Vcalhat}{\hat{\cV}}
\newcommand{\Wcalhat}{\hat{\cW}}
\newcommand{\Xcalhat}{\hat{\cX}}
\newcommand{\Ycalhat}{\hat{\cY}}
\newcommand{\Zcalhat}{\hat{\cZ}}

\newcommand{\cAhat}{\hat{\cA}}
\newcommand{\cBhat}{\hat{\cB}}
\newcommand{\cChat}{\hat{\cC}}
\newcommand{\cDhat}{\hat{\cD}}
\newcommand{\cEhat}{\hat{\cE}}
\newcommand{\cFhat}{\hat{\cF}}
\newcommand{\cGhat}{\hat{\cG}}
\newcommand{\cHhat}{\hat{\cH}}
\newcommand{\cIhat}{\hat{\cI}}
\newcommand{\cJhat}{\hat{\cJ}}
\newcommand{\cKhat}{\hat{\cK}}
\newcommand{\cLhat}{\hat{\cL}}
\newcommand{\cMhat}{\hat{\cM}}
\newcommand{\cNhat}{\hat{\cN}}
\newcommand{\cOhat}{\hat{\cO}}
\newcommand{\cPhat}{\hat{\cP}}
\newcommand{\cQhat}{\hat{\cQ}}
\newcommand{\cRhat}{\hat{\cR}}
\newcommand{\cShat}{\hat{\cS}}
\newcommand{\cThat}{\hat{\cT}}
\newcommand{\cUhat}{\hat{\cU}}
\newcommand{\cVhat}{\hat{\cV}}
\newcommand{\cWhat}{\hat{\cW}}
\newcommand{\cXhat}{\hat{\cX}}
\newcommand{\cYhat}{\hat{\cY}}
\newcommand{\cZhat}{\hat{\cZ}}

\newcommand{\Acalbar}{\bar{\cA}}
\newcommand{\Bcalbar}{\bar{\cB}}
\newcommand{\Ccalbar}{\bar{\cC}}
\newcommand{\Dcalbar}{\bar{\cD}}
\newcommand{\Ecalbar}{\bar{\cE}}
\newcommand{\Fcalbar}{\bar{\cF}}
\newcommand{\Gcalbar}{\bar{\cG}}
\newcommand{\Hcalbar}{\bar{\cH}}
\newcommand{\Icalbar}{\bar{\cI}}
\newcommand{\Jcalbar}{\bar{\cJ}}
\newcommand{\Kcalbar}{\bar{\cK}}
\newcommand{\Lcalbar}{\bar{\cL}}
\newcommand{\Mcalbar}{\bar{\cM}}
\newcommand{\Ncalbar}{\bar{\cN}}
\newcommand{\Ocalbar}{\bar{\cO}}
\newcommand{\Pcalbar}{\bar{\cP}}
\newcommand{\Qcalbar}{\bar{\cQ}}
\newcommand{\Rcalbar}{\bar{\cR}}
\newcommand{\Scalbar}{\bar{\cS}}
\newcommand{\Tcalbar}{\bar{\cT}}
\newcommand{\Ucalbar}{\bar{\cU}}
\newcommand{\Vcalbar}{\bar{\cV}}
\newcommand{\Wcalbar}{\bar{\cW}}
\newcommand{\Xcalbar}{\bar{\cX}}
\newcommand{\Ycalbar}{\bar{\cY}}
\newcommand{\Zcalbar}{\bar{\cZ}}

\newcommand{\cAbar}{\bar{\cA}}
\newcommand{\cBbar}{\bar{\cB}}
\newcommand{\cCbar}{\bar{\cC}}
\newcommand{\cDbar}{\bar{\cD}}
\newcommand{\cEbar}{\bar{\cE}}
\newcommand{\cFbar}{\bar{\cF}}
\newcommand{\cGbar}{\bar{\cG}}
\newcommand{\cHbar}{\bar{\cH}}
\newcommand{\cIbar}{\bar{\cI}}
\newcommand{\cJbar}{\bar{\cJ}}
\newcommand{\cKbar}{\bar{\cK}}
\newcommand{\cLbar}{\bar{\cL}}
\newcommand{\cMbar}{\bar{\cM}}
\newcommand{\cNbar}{\bar{\cN}}
\newcommand{\cObar}{\bar{\cO}}
\newcommand{\cPbar}{\bar{\cP}}
\newcommand{\cQbar}{\bar{\cQ}}
\newcommand{\cRbar}{\bar{\cR}}
\newcommand{\cSbar}{\bar{\cS}}
\newcommand{\cTbar}{\bar{\cT}}
\newcommand{\cUbar}{\bar{\cU}}
\newcommand{\cVbar}{\bar{\cV}}
\newcommand{\cWbar}{\bar{\cW}}
\newcommand{\cXbar}{\bar{\cX}}
\newcommand{\cYbar}{\bar{\cY}}
\newcommand{\cZbar}{\bar{\cZ}}

\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sE}{\mathscr{E}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sI}{\mathscr{I}}
\newcommand{\sJ}{\mathscr{J}}
\newcommand{\sK}{\mathscr{K}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sO}{\mathscr{O}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sQ}{\mathscr{Q}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\sS}{\mathscr{S}}
\newcommand{\sT}{\mathscr{T}}
\newcommand{\sU}{\mathscr{U}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sW}{\mathscr{W}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}

\newcommand{\sAbar}{\bar{\sA}}
\newcommand{\sBbar}{\bar{\sB}}
\newcommand{\sCbar}{\bar{\sC}}
\newcommand{\sDbar}{\bar{\sD}}
\newcommand{\sEbar}{\bar{\sE}}
\newcommand{\sFbar}{\bar{\sF}}
\newcommand{\sGbar}{\bar{\sG}}
\newcommand{\sHbar}{\bar{\sH}}
\newcommand{\sIbar}{\bar{\sI}}
\newcommand{\sJbar}{\bar{\sJ}}
\newcommand{\sKbar}{\bar{\sK}}
\newcommand{\sLbar}{\bar{\sL}}
\newcommand{\sMbar}{\bar{\sM}}
\newcommand{\sNbar}{\bar{\sN}}
\newcommand{\sObar}{\bar{\sO}}
\newcommand{\sPbar}{\bar{\sP}}
\newcommand{\sQbar}{\bar{\sQ}}
\newcommand{\sRbar}{\bar{\sR}}
\newcommand{\sSbar}{\bar{\sS}}
\newcommand{\sTbar}{\bar{\sT}}
\newcommand{\sUbar}{\bar{\sU}}
\newcommand{\sVbar}{\bar{\sV}}
\newcommand{\sWbar}{\bar{\sW}}
\newcommand{\sXbar}{\bar{\sX}}
\newcommand{\sYbar}{\bar{\sY}}
\newcommand{\sZbar}{\bar{\sZ}}

\newcommand{\sAhat}{\hat{\sA}}
\newcommand{\sBhat}{\hat{\sB}}
\newcommand{\sChat}{\hat{\sC}}
\newcommand{\sDhat}{\hat{\sD}}
\newcommand{\sEhat}{\hat{\sE}}
\newcommand{\sFhat}{\hat{\sF}}
\newcommand{\sGhat}{\hat{\sG}}
\newcommand{\sHhat}{\hat{\sH}}
\newcommand{\sIhat}{\hat{\sI}}
\newcommand{\sJhat}{\hat{\sJ}}
\newcommand{\sKhat}{\hat{\sK}}
\newcommand{\sLhat}{\hat{\sL}}
\newcommand{\sMhat}{\hat{\sM}}
\newcommand{\sNhat}{\hat{\sN}}
\newcommand{\sOhat}{\hat{\sO}}
\newcommand{\sPhat}{\hat{\sP}}
\newcommand{\sQhat}{\hat{\sQ}}
\newcommand{\sRhat}{\hat{\sR}}
\newcommand{\sShat}{\hat{\sS}}
\newcommand{\sThat}{\hat{\sT}}
\newcommand{\sUhat}{\hat{\sU}}
\newcommand{\sVhat}{\hat{\sV}}
\newcommand{\sWhat}{\hat{\sW}}
\newcommand{\sXhat}{\hat{\sX}}
\newcommand{\sYhat}{\hat{\sY}}
\newcommand{\sZhat}{\hat{\sZ}}

\newcommand{\sAtilde}{\widetilde{\sA}}
\newcommand{\sBtilde}{\widetilde{\sB}}
\newcommand{\sCtilde}{\widetilde{\sC}}
\newcommand{\sDtilde}{\widetilde{\sD}}
\newcommand{\sEtilde}{\widetilde{\sE}}
\newcommand{\sFtilde}{\widetilde{\sF}}
\newcommand{\sGtilde}{\widetilde{\sG}}
\newcommand{\sHtilde}{\widetilde{\sH}}
\newcommand{\sItilde}{\widetilde{\sI}}
\newcommand{\sJtilde}{\widetilde{\sJ}}
\newcommand{\sKtilde}{\widetilde{\sK}}
\newcommand{\sLtilde}{\widetilde{\sL}}
\newcommand{\sMtilde}{\widetilde{\sM}}
\newcommand{\sNtilde}{\widetilde{\sN}}
\newcommand{\sOtilde}{\widetilde{\sO}}
\newcommand{\sPtilde}{\widetilde{\sP}}
\newcommand{\sQtilde}{\widetilde{\sQ}}
\newcommand{\sRtilde}{\widetilde{\sR}}
\newcommand{\sStilde}{\widetilde{\sS}}
\newcommand{\sTtilde}{\widetilde{\sT}}
\newcommand{\sUtilde}{\widetilde{\sU}}
\newcommand{\sVtilde}{\widetilde{\sV}}
\newcommand{\sWtilde}{\widetilde{\sW}}
\newcommand{\sXtilde}{\widetilde{\sX}}
\newcommand{\sYtilde}{\widetilde{\sY}}
\newcommand{\sZtilde}{\widetilde{\sZ}}

\newcommand{\sAt}{\tilde{\sA}}
\newcommand{\sBt}{\tilde{\sB}}
\newcommand{\sCt}{\tilde{\sC}}
\newcommand{\sDt}{\tilde{\sD}}
\newcommand{\sEt}{\tilde{\sE}}
\newcommand{\sFt}{\tilde{\sF}}
\newcommand{\sGt}{\tilde{\sG}}
\newcommand{\sHt}{\tilde{\sH}}
\newcommand{\sIt}{\tilde{\sI}}
\newcommand{\sJt}{\tilde{\sJ}}
\newcommand{\sKt}{\tilde{\sK}}
\newcommand{\sLt}{\tilde{\sL}}
\newcommand{\sMt}{\tilde{\sM}}
\newcommand{\sNt}{\tilde{\sN}}
\newcommand{\sOt}{\tilde{\sO}}
\newcommand{\sPt}{\tilde{\sP}}
\newcommand{\sQt}{\tilde{\sQ}}
\newcommand{\sRt}{\tilde{\sR}}
\newcommand{\sSt}{\tilde{\sS}}
\newcommand{\sTt}{\tilde{\sT}}
\newcommand{\sUt}{\tilde{\sU}}
\newcommand{\sVt}{\tilde{\sV}}
\newcommand{\sWt}{\tilde{\sW}}
\newcommand{\sXt}{\tilde{\sX}}
\newcommand{\sYt}{\tilde{\sY}}
\newcommand{\sZt}{\tilde{\sZ}}

\newcommand{\dA}{\mathds{A}}
\newcommand{\dB}{\mathds{B}}
\newcommand{\dC}{\mathds{C}}
\newcommand{\dD}{\mathds{D}}
\newcommand{\dE}{\mathds{E}}
\newcommand{\dF}{\mathds{F}}
\newcommand{\dG}{\mathds{G}}
\newcommand{\dH}{\mathds{H}}
\newcommand{\dI}{\mathds{I}}
\newcommand{\dJ}{\mathds{J}}
\newcommand{\dK}{\mathds{K}}
\newcommand{\dL}{\mathds{L}}
\newcommand{\dM}{\mathds{M}}
\newcommand{\dN}{\mathds{N}}
\newcommand{\dO}{\mathds{O}}
\newcommand{\dP}{\mathds{P}}
\newcommand{\dQ}{\mathds{Q}}
\newcommand{\dR}{\mathds{R}}
\newcommand{\dS}{\mathds{S}}
\newcommand{\dT}{\mathds{T}}
\newcommand{\dU}{\mathds{U}}
\newcommand{\dV}{\mathds{V}}
\newcommand{\dW}{\mathds{W}}
\newcommand{\dX}{\mathds{X}}
\newcommand{\dY}{\mathds{Y}}
\newcommand{\dZ}{\mathds{Z}}

\newcommand{\dAbar}{\bar{\dA}}
\newcommand{\dBbar}{\bar{\dB}}
\newcommand{\dCbar}{\bar{\dC}}
\newcommand{\dDbar}{\bar{\dD}}
\newcommand{\dEbar}{\bar{\dE}}
\newcommand{\dFbar}{\bar{\dF}}
\newcommand{\dGbar}{\bar{\dG}}
\newcommand{\dHbar}{\bar{\dH}}
\newcommand{\dIbar}{\bar{\dI}}
\newcommand{\dJbar}{\bar{\dJ}}
\newcommand{\dKbar}{\bar{\dK}}
\newcommand{\dLbar}{\bar{\dL}}
\newcommand{\dMbar}{\bar{\dM}}
\newcommand{\dNbar}{\bar{\dN}}
\newcommand{\dObar}{\bar{\dO}}
\newcommand{\dPbar}{\bar{\dP}}
\newcommand{\dQbar}{\bar{\dQ}}
\newcommand{\dRbar}{\bar{\dR}}
\newcommand{\dSbar}{\bar{\dS}}
\newcommand{\dTbar}{\bar{\dT}}
\newcommand{\dUbar}{\bar{\dU}}
\newcommand{\dVbar}{\bar{\dV}}
\newcommand{\dWbar}{\bar{\dW}}
\newcommand{\dXbar}{\bar{\dX}}
\newcommand{\dYbar}{\bar{\dY}}
\newcommand{\dZbar}{\bar{\dZ}}

\newcommand{\dAhat}{\hat{\dA}}
\newcommand{\dBhat}{\hat{\dB}}
\newcommand{\dChat}{\hat{\dC}}
\newcommand{\dDhat}{\hat{\dD}}
\newcommand{\dEhat}{\hat{\dE}}
\newcommand{\dFhat}{\hat{\dF}}
\newcommand{\dGhat}{\hat{\dG}}
\newcommand{\dHhat}{\hat{\dH}}
\newcommand{\dIhat}{\hat{\dI}}
\newcommand{\dJhat}{\hat{\dJ}}
\newcommand{\dKhat}{\hat{\dK}}
\newcommand{\dLhat}{\hat{\dL}}
\newcommand{\dMhat}{\hat{\dM}}
\newcommand{\dNhat}{\hat{\dN}}
\newcommand{\dOhat}{\hat{\dO}}
\newcommand{\dPhat}{\hat{\dP}}
\newcommand{\dQhat}{\hat{\dQ}}
\newcommand{\dRhat}{\hat{\dR}}
\newcommand{\dShat}{\hat{\dS}}
\newcommand{\dThat}{\hat{\dT}}
\newcommand{\dUhat}{\hat{\dU}}
\newcommand{\dVhat}{\hat{\dV}}
\newcommand{\dWhat}{\hat{\dW}}
\newcommand{\dXhat}{\hat{\dX}}
\newcommand{\dYhat}{\hat{\dY}}
\newcommand{\dZhat}{\hat{\dZ}}

\newcommand{\dAtilde}{\widetilde{\dA}}
\newcommand{\dBtilde}{\widetilde{\dB}}
\newcommand{\dCtilde}{\widetilde{\dC}}
\newcommand{\dDtilde}{\widetilde{\dD}}
\newcommand{\dEtilde}{\widetilde{\dE}}
\newcommand{\dFtilde}{\widetilde{\dF}}
\newcommand{\dGtilde}{\widetilde{\dG}}
\newcommand{\dHtilde}{\widetilde{\dH}}
\newcommand{\dItilde}{\widetilde{\dI}}
\newcommand{\dJtilde}{\widetilde{\dJ}}
\newcommand{\dKtilde}{\widetilde{\dK}}
\newcommand{\dLtilde}{\widetilde{\dL}}
\newcommand{\dMtilde}{\widetilde{\dM}}
\newcommand{\dNtilde}{\widetilde{\dN}}
\newcommand{\dOtilde}{\widetilde{\dO}}
\newcommand{\dPtilde}{\widetilde{\dP}}
\newcommand{\dQtilde}{\widetilde{\dQ}}
\newcommand{\dRtilde}{\widetilde{\dR}}
\newcommand{\dStilde}{\widetilde{\dS}}
\newcommand{\dTtilde}{\widetilde{\dT}}
\newcommand{\dUtilde}{\widetilde{\dU}}
\newcommand{\dVtilde}{\widetilde{\dV}}
\newcommand{\dWtilde}{\widetilde{\dW}}
\newcommand{\dXtilde}{\widetilde{\dX}}
\newcommand{\dYtilde}{\widetilde{\dY}}
\newcommand{\dZtilde}{\widetilde{\dZ}}

\newcommand{\dAt}{\tilde{\dA}}
\newcommand{\dBt}{\tilde{\dB}}
\newcommand{\dCt}{\tilde{\dC}}
\newcommand{\dDt}{\tilde{\dD}}
\newcommand{\dEt}{\tilde{\dE}}
\newcommand{\dFt}{\tilde{\dF}}
\newcommand{\dGt}{\tilde{\dG}}
\newcommand{\dHt}{\tilde{\dH}}
\newcommand{\dIt}{\tilde{\dI}}
\newcommand{\dJt}{\tilde{\dJ}}
\newcommand{\dKt}{\tilde{\dK}}
\newcommand{\dLt}{\tilde{\dL}}
\newcommand{\dMt}{\tilde{\dM}}
\newcommand{\dNt}{\tilde{\dN}}
\newcommand{\dOt}{\tilde{\dO}}
\newcommand{\dPt}{\tilde{\dP}}
\newcommand{\dQt}{\tilde{\dQ}}
\newcommand{\dRt}{\tilde{\dR}}
\newcommand{\dSt}{\tilde{\dS}}
\newcommand{\dTt}{\tilde{\dT}}
\newcommand{\dUt}{\tilde{\dU}}
\newcommand{\dVt}{\tilde{\dV}}
\newcommand{\dWt}{\tilde{\dW}}
\newcommand{\dXt}{\tilde{\dX}}
\newcommand{\dYt}{\tilde{\dY}}
\newcommand{\dZt}{\tilde{\dZ}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\ve}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vj}{\vec{j}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vl}{\vec{l}}
\newcommand{\vm}{\vec{m}}
\newcommand{\vn}{\vec{n}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}
\newcommand{\VV}{\mathrm{Var}}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}




\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  %
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\Proof\undefined
\newcommand{\Proof}{\noindent{\bf Proof.}~}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi




\newcommand{\done}{\mathds{1}} %
\newcommand{\dAA}{\mathds{A}} 
\newcommand{\BB}{\mathds{B}} 
\newcommand{\CC}{\mathds{C}} %
\newcommand{\DD}{\mathds{D}} 
\newcommand{\EE}{\mathds{E}} %
\newcommand{\FF}{\mathds{F}} %
\newcommand{\GG}{\mathds{G}} 
\newcommand{\HH}{\mathds{H}} %
\newcommand{\II}{\mathds{I}} %
\newcommand{\JJ}{\mathds{J}} 
\newcommand{\KK}{\mathds{K}} %
\newcommand{\LL}{\mathds{L}} 
\newcommand{\MM}{\mathds{M}} %
\newcommand{\NN}{\mathbb{N}} %
\newcommand{\OO}{\mathds{O}} 
\newcommand{\PP}{\mathds{P}} %
\newcommand{\QQ}{\mathds{Q}} %
\newcommand{\RR}{\mathbb{R}} %
\newcommand{\dSS}{\mathbb{S}} 
\newcommand{\RRbar}{\overline{\RR}} %
\newcommand{\TT}{\mathds{T}} 
\newcommand{\UU}{\mathds{U}} 
\newcommand{\WW}{\mathds{W}} 
\newcommand{\XX}{\mathds{X}}
\newcommand{\YY}{\mathds{Y}}
\newcommand{\ZZ}{\mathds{Z}} %


\newcommand*{\mini}{\operatorname*{minimize}}
\newcommand*{\maxi}{\operatorname*{maximize}}
\newcommand*{\argmin}{\operatorname*{argmin}}
\newcommand*{\argmax}{\operatorname*{argmax}}
\newcommand*{\arginf}{\operatorname*{arginf}}
\newcommand*{\argsup}{\operatorname*{argsup}}

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

\newcommand{\co}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{co}\else\operatorname{co}\left(#1\right)\fi}
\newcommand{\core}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{core}\else\operatorname{core}\left(#1\right)\fi}
\newcommand{\diag}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{diag}\else\operatorname{diag}\left(#1\right)\fi}
\newcommand{\dom}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{dom}\else\operatorname{dom}\left(#1\right)\fi}
\newcommand{\expect}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathds{E}}\else\operatorname{\mathds{E}}\ssbr{#1}\fi}
\newcommand{\lap}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\bf Lap}\else\operatorname{\bf Lap}\left(#1\right)\fi}
\newcommand{\prob}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathds{P}}\else\operatorname{\mathds{P}}\ssbr{#1}\fi}
\newcommand{\proj}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathcal{P}}\else\operatorname{\mathcal{P}}\left(#1\right)\fi}
\newcommand{\prox}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{prox}\else\operatorname{prox}\left(#1\right)\fi}
\newcommand{\sgn}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{sign}\else\operatorname{sign}\left(#1\right)\fi}
\newcommand{\sign}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{sign}\else\operatorname{sign}\left(#1\right)\fi}
\newcommand{\traj}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{Traj}\else\operatorname{Traj}\left(#1\right)\fi}
\newcommand{\vect}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{vec}\else\operatorname{vec}\left(#1\right)\fi}

\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\ri}{\operatorname{ri}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\intr}{\operatorname{int}}
\newcommand{\emp}{\operatorname{emp}}
\newcommand{\nnz}{\operatorname{nnz}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}
\renewcommand{\O}{{\cO}}
\newcommand{\softO}[1]{{\widetilde{\cO}}\rbr{#1}}

\newcommand{\Co}[1]{\co[#1]}
\newcommand{\Core}[1]{\core[#1]}
\newcommand{\Diag}[1]{\diag[#1]}
\newcommand{\Dom}[1]{\dom[#1]}
\newcommand{\Expect}[2][]{\underset{#1}{\EE}\ssbr{{#2}}}
\newcommand{\Ind}[1]{\ind[#1]}
\newcommand{\Lap}[1]{\lap[#1]}
\newcommand{\Prob}[1]{\prob[#1]}
\newcommand{\Proj}[2][]{\mathcal{P}_{#1}\sbr{#2}}
\newcommand{\Prox}[2][]{\operatorname{prox}_{#1}\rbr{#2}}
\newcommand{\Rank}[1]{\rank[#1]}
\newcommand{\Sgn}[1]{\sgn[#1]}
\newcommand{\Sign}[1]{\sign[#1]}
\newcommand{\Traj}[1]{\traj[#1]}
\newcommand{\Vect}[1]{\vect[#1]}


\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}


\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}


\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }


\newcommand{\rbr}[1]{\left({#1}\right)}
\newcommand{\sbr}[1]{\left[{#1}\right]}
\newcommand{\cbr}[1]{\left\{{#1}\right\}}
\newcommand{\nbr}[1]{\left\|{#1}\right\|}
\newcommand{\abr}[1]{\left\langle{#1}\right\rangle}
\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\inner}[2]{\left\langle {#1},{#2} \right\rangle}
\newcommand{\frob}[1]{\norm{#1}_\text{F}}
\newcommand{\fro}[1]{\norm{#1}_\text{F}}
\newcommand{\onenorm}[1]{\norm{#1}_1}
\newcommand{\twonorm}[1]{\norm{#1}_2}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\trnorm}[1]{\norm{#1}_{\text{tr}}}
\newcommand{\ccc}[1]{\left|\!\left|\!\left|{#1}\right|\!\right|\!\right|}
\newcommand{\bsd}[1]{\left\llbracket{#1}\right\rrbracket}
\newcommand{\ssbr}[1]{\left\llbracket{#1}\right\rrbracket}
\newcommand{\sembrack}[1]{\left\llbracket{#1}\right\rrbracket}


\newcommand{\one}{{\bm{1}}}  %
\newcommand{\zero}{{\bm{0}}} %
\newcommand{\bone}{{\bm{1}}}  %
\newcommand{\bzero}{{\bm{0}}} %
\def\b0{\bm{0}} %
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}
\newcommand*{\diff}[1][]{\mathop{}\!{\mathrm{d}^{#1}}}


\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\valpha}{\vec{\alpha}}
\newcommand{\AL}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vgamma}{\vec{\gamma}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vdelta}{\vec{\delta}}
\newcommand{\veps}{\vec{\epsilon}}
\newcommand{\vepsilon}{\vec{\epsilon}}
\newcommand{\vze}{\vec{\zeta}}
\newcommand{\vzeta}{\vec{\zeta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\vtheta}{\vec{\theta}}
\newcommand{\viota}{\vec{\iota}}
\newcommand{\vkappa}{\vec{\kappa}}
\newcommand{\vlambda}{\vec{\lambda}}
\newcommand{\vmu}{\vec{\mu}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vrho}{\vec{\rho}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vsigma}{\vec{\sigma}}
\newcommand{\vtau}{\vec{\tau}}
\newcommand{\vupsilon}{\vec{\upsilon}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vchi}{\vec{\chi}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vomega}{\vec{\omega}}

\newcommand{\bal}{\vec{\alpha}}
\newcommand{\balpha}{\vec{\alpha}}
\newcommand{\bbeta}{\vec{\beta}}
\newcommand{\bga}{\vec{\gamma}}
\newcommand{\bgamma}{\vec{\gamma}}
\newcommand{\bde}{\vec{\delta}}
\newcommand{\bdelta}{\vec{\delta}}
\newcommand{\beps}{\vec{\epsilon}}
\newcommand{\bepsilon}{\vec{\epsilon}}
\newcommand{\bze}{\vec{\zeta}}
\newcommand{\bzeta}{\vec{\zeta}}
\newcommand{\boldeta}{\vec{\eta}}
\newcommand{\bth}{\vec{\theta}}
\newcommand{\btheta}{\vec{\theta}}
\newcommand{\biota}{\vec{\iota}}
\newcommand{\bkappa}{\vec{\kappa}}
\newcommand{\blambda}{\vec{\lambda}}
\newcommand{\bmu}{\vec{\mu}}
\newcommand{\bnu}{\vec{\nu}}
\newcommand{\bxi}{\vec{\xi}}
\newcommand{\bpi}{\vec{\pi}}
\newcommand{\brho}{\vec{\rho}}
\newcommand{\bsig}{\vec{\sigma}}
\newcommand{\bsigma}{\vec{\sigma}}
\newcommand{\btau}{\vec{\tau}}
\newcommand{\bupsilon}{\vec{\upsilon}}
\newcommand{\bphi}{\vec{\phi}}
\newcommand{\bchi}{\vec{\chi}}
\newcommand{\bpsi}{\vec{\psi}}
\newcommand{\bomega}{\vec{\omega}}

\newcommand{\ALbar}{\bar{\val}}
\newcommand{\balbar}{\bar{\val}}
\newcommand{\balphabar}{\bar{\val}}
\newcommand{\bbetabar}{\bar{\vbeta}}
\newcommand{\bgabar}{\bar{\vgamma}}
\newcommand{\bgammabar}{\bar{\vgamma}}
\newcommand{\bdebar}{\bar{\vdelta}}
\newcommand{\bdeltabar}{\bar{\vdelta}}
\newcommand{\bepsbar}{\bar{\vepsilon}}
\newcommand{\bepsilonbar}{\bar{\vepsilon}}
\newcommand{\bzebar}{\bar{\vzeta}}
\newcommand{\bzetabar}{\bar{\vzeta}}
\newcommand{\boldetabar}{\bar{\veta}}
\newcommand{\bthbar}{\bar{\vtheta}}
\newcommand{\bthetabar}{\bar{\vtheta}}
\newcommand{\biotabar}{\bar{\viota}}
\newcommand{\bkappabar}{\bar{\vkappa}}
\newcommand{\blambdabar}{\bar{\vlambda}}
\newcommand{\bmubar}{\bar{\vmu}}
\newcommand{\bnubar}{\bar{\vnu}}
\newcommand{\bxibar}{\bar{\vxi}}
\newcommand{\bpibar}{\bar{\vpi}}
\newcommand{\brhobar}{\bar{\vrho}}
\newcommand{\bsigbar}{\bar{\vsigma}}
\newcommand{\bsigmabar}{\bar{\vsigma}}
\newcommand{\btaubar}{\bar{\vtau}}
\newcommand{\bupsilonbar}{\bar{\vupsilon}}
\newcommand{\bphibar}{\bar{\vphi}}
\newcommand{\bchibar}{\bar{\vchi}}
\newcommand{\bpsibar}{\bar{\vpsi}}
\newcommand{\bomegabar}{\bar{\vomega}}

\newcommand{\ALhat}{\hat{\val}}
\newcommand{\balhat}{\hat{\val}}
\newcommand{\balphahat}{\hat{\val}}
\newcommand{\bbetahat}{\hat{\vbeta}}
\newcommand{\bgahat}{\hat{\vgamma}}
\newcommand{\bgammahat}{\hat{\vgamma}}
\newcommand{\bdehat}{\hat{\vdelta}}
\newcommand{\bdeltahat}{\hat{\vdelta}}
\newcommand{\bepshat}{\hat{\vepsilon}}
\newcommand{\bepsilonhat}{\hat{\vepsilon}}
\newcommand{\bzehat}{\hat{\vzeta}}
\newcommand{\bzetahat}{\hat{\vzeta}}
\newcommand{\boldetahat}{\hat{\veta}}
\newcommand{\bthhat}{\hat{\vtheta}}
\newcommand{\bthetahat}{\hat{\vtheta}}
\newcommand{\biotahat}{\hat{\viota}}
\newcommand{\bkappahat}{\hat{\vkappa}}
\newcommand{\blambdahat}{\hat{\vlambda}}
\newcommand{\bmuhat}{\hat{\vmu}}
\newcommand{\bnuhat}{\hat{\vnu}}
\newcommand{\bxihat}{\hat{\vxi}}
\newcommand{\bpihat}{\hat{\vpi}}
\newcommand{\brhohat}{\hat{\vrho}}
\newcommand{\bsighat}{\hat{\vsigma}}
\newcommand{\bsigmahat}{\hat{\vsigma}}
\newcommand{\btauhat}{\hat{\vtau}}
\newcommand{\bupsilonhat}{\hat{\vupsilon}}
\newcommand{\bphihat}{\hat{\vphi}}
\newcommand{\bchihat}{\hat{\vchi}}
\newcommand{\bpsihat}{\hat{\vpsi}}
\newcommand{\bomegahat}{\hat{\vomega}}

\newcommand{\ALtil}{\tilde{\val}}
\newcommand{\baltil}{\tilde{\val}}
\newcommand{\balphatil}{\tilde{\val}}
\newcommand{\bbetatil}{\tilde{\vbeta}}
\newcommand{\bgatil}{\tilde{\vgamma}}
\newcommand{\bgammatil}{\tilde{\vgamma}}
\newcommand{\bdetil}{\tilde{\vdelta}}
\newcommand{\bdeltatil}{\tilde{\vdelta}}
\newcommand{\bepstil}{\tilde{\vepsilon}}
\newcommand{\bepsilontil}{\tilde{\vepsilon}}
\newcommand{\bzetil}{\tilde{\vzeta}}
\newcommand{\bzetatil}{\tilde{\vzeta}}
\newcommand{\boldetatil}{\tilde{\veta}}
\newcommand{\bthtil}{\tilde{\vtheta}}
\newcommand{\bthetatil}{\tilde{\vtheta}}
\newcommand{\biotatil}{\tilde{\viota}}
\newcommand{\bkappatil}{\tilde{\vkappa}}
\newcommand{\blambdatil}{\tilde{\vlambda}}
\newcommand{\bmutil}{\tilde{\vmu}}
\newcommand{\bnutil}{\tilde{\vnu}}
\newcommand{\bxitil}{\tilde{\vxi}}
\newcommand{\bpitil}{\tilde{\vpi}}
\newcommand{\brhotil}{\tilde{\vrho}}
\newcommand{\bsigtil}{\tilde{\vsigma}}
\newcommand{\bsigmatil}{\tilde{\vsigma}}
\newcommand{\btautil}{\tilde{\vtau}}
\newcommand{\bupsilontil}{\tilde{\vupsilon}}
\newcommand{\bphitil}{\tilde{\vphi}}
\newcommand{\bchitil}{\tilde{\vchi}}
\newcommand{\bpsitil}{\tilde{\vpsi}}
\newcommand{\bomegatil}{\tilde{\vomega}}

\newcommand{\ALtilde}{\widetilde{\val}}
\newcommand{\baltilde}{\widetilde{\val}}
\newcommand{\balphatilde}{\widetilde{\val}}
\newcommand{\bbetatilde}{\widetilde{\vbeta}}
\newcommand{\bgatilde}{\widetilde{\vgamma}}
\newcommand{\bgammatilde}{\widetilde{\vgamma}}
\newcommand{\bdetilde}{\widetilde{\vdelta}}
\newcommand{\bdeltatilde}{\widetilde{\vdelta}}
\newcommand{\bepstilde}{\widetilde{\vepsilon}}
\newcommand{\bepsilontilde}{\widetilde{\vepsilon}}
\newcommand{\bzetilde}{\widetilde{\vzeta}}
\newcommand{\bzetatilde}{\widetilde{\vzeta}}
\newcommand{\boldetatilde}{\widetilde{\veta}}
\newcommand{\bthtilde}{\widetilde{\vtheta}}
\newcommand{\bthetatilde}{\widetilde{\vtheta}}
\newcommand{\biotatilde}{\widetilde{\viota}}
\newcommand{\bkappatilde}{\widetilde{\vkappa}}
\newcommand{\blambdatilde}{\widetilde{\vlambda}}
\newcommand{\bmutilde}{\widetilde{\vmu}}
\newcommand{\bnutilde}{\widetilde{\vnu}}
\newcommand{\bxitilde}{\widetilde{\vxi}}
\newcommand{\bpitilde}{\widetilde{\vpi}}
\newcommand{\brhotilde}{\widetilde{\vrho}}
\newcommand{\bsigtilde}{\widetilde{\vsigma}}
\newcommand{\bsigmatilde}{\widetilde{\vsigma}}
\newcommand{\btautilde}{\widetilde{\vtau}}
\newcommand{\bupsilontilde}{\widetilde{\vupsilon}}
\newcommand{\bphitilde}{\widetilde{\vphi}}
\newcommand{\bchitilde}{\widetilde{\vchi}}
\newcommand{\bpsitilde}{\widetilde{\vpsi}}
\newcommand{\bomegatilde}{\widetilde{\vomega}}

\newcommand{\ALt}{\tilde{\val}}
\newcommand{\balt}{\tilde{\val}}
\newcommand{\balphat}{\hat{\val}}
\newcommand{\bbetat}{\tilde{\vbeta}}
\newcommand{\bgat}{\tilde{\vgamma}}
\newcommand{\bgammat}{\tilde{\vgamma}}
\newcommand{\bdet}{\tilde{\vdelta}}
\newcommand{\bdeltat}{\tilde{\vdelta}}
\newcommand{\bepst}{\tilde{\vepsilon}}
\newcommand{\bepsilont}{\tilde{\vepsilon}}
\newcommand{\bzet}{\tilde{\vzeta}}
\newcommand{\bzetat}{\tilde{\vzeta}}
\newcommand{\boldetat}{\tilde{\veta}}
\newcommand{\btht}{\tilde{\vtheta}}
\newcommand{\bthetat}{\tilde{\vtheta}}
\newcommand{\biotat}{\tilde{\viota}}
\newcommand{\bkappat}{\tilde{\vkappa}}
\newcommand{\blambdat}{\tilde{\vlambda}}
\newcommand{\bmut}{\tilde{\vmu}}
\newcommand{\bnut}{\tilde{\vnu}}
\newcommand{\bxit}{\tilde{\vxi}}
\newcommand{\bpit}{\tilde{\vpi}}
\newcommand{\brhot}{\tilde{\vrho}}
\newcommand{\bsigt}{\tilde{\vsigma}}
\newcommand{\bsigmat}{\tilde{\vsigma}}
\newcommand{\btaut}{\tilde{\vtau}}
\newcommand{\bupsilont}{\tilde{\vupsilon}}
\newcommand{\bphit}{\tilde{\vphi}}
\newcommand{\bchit}{\tilde{\vchi}}
\newcommand{\bpsit}{\tilde{\vpsi}}
\newcommand{\bomegat}{\tilde{\vomega}}

\newcommand{\albar}{\bar{\al}}
\newcommand{\alphabar}{\bar{\al}}
\newcommand{\betabar}{\bar{\beta}}
\newcommand{\gabar}{\bar{\gamma}}
\newcommand{\gammabar}{\bar{\gamma}}
\newcommand{\debar}{\bar{\delta}}
\newcommand{\deltabar}{\bar{\delta}}
\newcommand{\epsbar}{\bar{\epsilon}}
\newcommand{\epsilonbar}{\bar{\epsilon}}
\newcommand{\zebar}{\bar{\zeta}}
\newcommand{\zetabar}{\bar{\zeta}}
\newcommand{\etabar}{\bar{\eta}}
\newcommand{\thbar}{\bar{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\iotabar}{\bar{\iota}}
\newcommand{\kappabar}{\bar{\kappa}}
\newcommand{\lambdabar}{\bar{\lambda}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\xibar}{\bar{\xi}}
\newcommand{\pibar}{\bar{\pi}}
\newcommand{\rhobar}{\bar{\rho}}
\newcommand{\sigbar}{\bar{\sigma}}
\newcommand{\sigmabar}{\bar{\sigma}}
\newcommand{\taubar}{\bar{\tau}}
\newcommand{\upsilonbar}{\bar{\upsilon}}
\newcommand{\phibar}{\bar{\phi}}
\newcommand{\chibar}{\bar{\chi}}
\newcommand{\psibar}{\bar{\psi}}
\newcommand{\omegabar}{\bar{\omega}}

\newcommand{\alhat}{\hat{\al}}
\newcommand{\alphahat}{\hat{\al}}
\newcommand{\betahat}{\hat{\beta}}
\newcommand{\gahat}{\hat{\gamma}}
\newcommand{\gammahat}{\hat{\gamma}}
\newcommand{\dehat}{\hat{\delta}}
\newcommand{\deltahat}{\hat{\delta}}
\newcommand{\epshat}{\hat{\epsilon}}
\newcommand{\epsilonhat}{\hat{\epsilon}}
\newcommand{\zehat}{\hat{\zeta}}
\newcommand{\zetahat}{\hat{\zeta}}
\newcommand{\etahat}{\hat{\eta}}
\newcommand{\thhat}{\hat{\theta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\iotahat}{\hat{\iota}}
\newcommand{\kappahat}{\hat{\kappa}}
\newcommand{\lambdahat}{\hat{\lambda}}
\newcommand{\muhat}{\hat{\mu}}
\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\xihat}{\hat{\xi}}
\newcommand{\pihat}{\hat{\pi}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\sighat}{\hat{\sigma}}
\newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\tauhat}{\hat{\tau}}
\newcommand{\upsilonhat}{\hat{\upsilon}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\chihat}{\hat{\chi}}
\newcommand{\psihat}{\hat{\psi}}
\newcommand{\omegahat}{\hat{\omega}}

\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\betatil}{\tilde{\beta}}
\newcommand{\gatil}{\tilde{\gamma}}
\newcommand{\gammatil}{\tilde{\gamma}}
\newcommand{\deltatil}{\tilde{\delta}}
\newcommand{\epstil}{\tilde{\epsilon}}
\newcommand{\epsilontil}{\tilde{\epsilon}}
\newcommand{\zetil}{\tilde{\zeta}}
\newcommand{\zetatil}{\tilde{\zeta}}
\newcommand{\etatil}{\tilde{\eta}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\iotatil}{\tilde{\iota}}
\newcommand{\kappatil}{\tilde{\kappa}}
\newcommand{\lambdatil}{\tilde{\lambda}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\nutil}{\tilde{\nu}}
\newcommand{\xitil}{\tilde{\xi}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\rhotil}{\tilde{\rho}}
\newcommand{\sigtil}{\tilde{\sigma}}
\newcommand{\sigmatil}{\tilde{\sigma}}
\newcommand{\tautil}{\tilde{\tau}}
\newcommand{\upsilontil}{\tilde{\upsilon}}
\newcommand{\phitil}{\tilde{\phi}}
\newcommand{\chitil}{\tilde{\chi}}
\newcommand{\psitil}{\tilde{\psi}}
\newcommand{\omegatil}{\tilde{\omega}}

\newcommand{\alphat}{\tilde{\alpha}}
\newcommand{\betat}{\tilde{\beta}}
\newcommand{\gammat}{\tilde{\gamma}}
\newcommand{\deltat}{\tilde{\delta}}
\newcommand{\epsilont}{\tilde{\epsilon}}
\newcommand{\epst}{\tilde{\epsilon}}
\newcommand{\zetat}{\tilde{\zeta}}
\newcommand{\etat}{\tilde{\eta}}
\newcommand{\thetat}{\tilde{\theta}}
\newcommand{\iotat}{\tilde{\iota}}
\newcommand{\kappat}{\tilde{\kappa}}
\newcommand{\lambdat}{\tilde{\lambda}}
\newcommand{\mut}{\tilde{\mu}}
\newcommand{\nut}{\tilde{\nu}}
\newcommand{\xit}{\tilde{\xi}}
\newcommand{\pit}{\tilde{\pi}}
\newcommand{\rhot}{\tilde{\rho}}
\newcommand{\sigt}{\tilde{\sigma}}
\newcommand{\sigmat}{\tilde{\sigma}}
\newcommand{\taut}{\tilde{\tau}}
\newcommand{\upsilont}{\tilde{\upsilon}}
\newcommand{\phit}{\tilde{\phi}}
\newcommand{\chit}{\tilde{\chi}}
\newcommand{\psit}{\tilde{\psi}}
\newcommand{\omegat}{\tilde{\omega}}

\newcommand{\Gammabar}{\bar{\Gamma}}
\newcommand{\Deltabar}{\bar{\Delta}}
\newcommand{\Thetabar}{\bar{\Theta}}
\newcommand{\Lambdabar}{\bar{\Lambda}}
\newcommand{\Xibar}{\bar{\Xi}}
\newcommand{\Pibar}{\bar{\Pi}}
\newcommand{\Sigmabar}{\bar{\Sigma}}
\newcommand{\Upsilonbar}{\bar{\Upsilon}}
\newcommand{\Phibar}{\bar{\Phi}}
\newcommand{\Psibar}{\bar{\Psi}}
\newcommand{\Omegabar}{\bar{\Omega}}

\newcommand{\Gammahat}{\hat{\Gamma}}
\newcommand{\Deltahat}{\hat{\Delta}}
\newcommand{\Thetahat}{\hat{\Theta}}
\newcommand{\Lambdahat}{\hat{\Lambda}}
\newcommand{\Xihat}{\hat{\Xi}}
\newcommand{\Pihat}{\hat{\Pi}}
\newcommand{\Sigmahat}{\hat{\Sigma}}
\newcommand{\Upsilonhat}{\hat{\Upsilon}}
\newcommand{\Phihat}{\hat{\Phi}}
\newcommand{\Psihat}{\hat{\Psi}}
\newcommand{\Omegahat}{\hat{\Omega}}

\newcommand{\Gammatil}{\tilde{\Gamma}}
\newcommand{\Deltatil}{\tilde{\Delta}}
\newcommand{\Thetatil}{\tilde{\Theta}}
\newcommand{\Lambdatil}{\tilde{\Lambda}}
\newcommand{\Xitil}{\tilde{\Xi}}
\newcommand{\Pitil}{\tilde{\Pi}}
\newcommand{\Sigmatil}{\tilde{\Sigma}}
\newcommand{\Upsilontil}{\tilde{\Upsilon}}
\newcommand{\Phitil}{\tilde{\Phi}}
\newcommand{\Psitil}{\tilde{\Psi}}
\newcommand{\Omegatil}{\tilde{\Omega}}

\newcommand{\Gammatilde}{\widetilde{\Gamma}}
\newcommand{\Deltatilde}{\widetilde{\Delta}}
\newcommand{\Thetatilde}{\widetilde{\Theta}}
\newcommand{\Lambdatilde}{\widetilde{\Lambda}}
\newcommand{\Xitilde}{\widetilde{\Xi}}
\newcommand{\Pitilde}{\widetilde{\Pi}}
\newcommand{\Sigmatilde}{\widetilde{\Sigma}}
\newcommand{\Upsilontilde}{\widetilde{\Upsilon}}
\newcommand{\Phitilde}{\widetilde{\Phi}}
\newcommand{\Psitilde}{\widetilde{\Psi}}
\newcommand{\Omegatilde}{\widetilde{\Omega}}

\newcommand{\Gammat}{\tilde{\Gamma}}
\newcommand{\Deltat}{\tilde{\Delta}}
\newcommand{\Thetat}{\tilde{\Theta}}
\newcommand{\Lambdat}{\tilde{\Lambda}}
\newcommand{\Xit}{\tilde{\Xi}}
\newcommand{\Pit}{\tilde{\Pi}}
\newcommand{\Sigmat}{\tilde{\Sigma}}
\newcommand{\Upsilont}{\tilde{\Upsilon}}
\newcommand{\Phit}{\tilde{\Phi}}
\newcommand{\Psit}{\tilde{\Psi}}
\newcommand{\Omegat}{\tilde{\Omega}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\epsilonb}{\boldsymbol{\epsilon}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\delbar}{\bar{\delta}}

\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}



\newcommand{\Poisson}{\mathrm{Poisson}}

